Sample Complexity of Forecast Aggregation

We consider a Bayesian forecast aggregation model where $n$ experts, after observing private signals about an unknown binary event, report their posterior beliefs about the event to a principal, who then aggregates the reports into a single prediction for the event. The signals of the experts and the outcome of the event follow a joint distribution that is unknown to the principal, but the principal has access to i.i.d. "samples" from the distribution, where each sample is a tuple of the experts' reports (not signals) and the realization of the event. Using these samples, the principal aims to find an $\varepsilon$-approximately optimal aggregator, where optimality is measured in terms of the expected squared distance between the aggregated prediction and the realization of the event. We show that the sample complexity of this problem is at least $\tilde \Omega(m^{n-2} / \varepsilon)$ for arbitrary discrete distributions, where $m$ is the size of each expert's signal space. This sample complexity grows exponentially in the number of experts $n$. But, if the experts' signals are independent conditioned on the realization of the event, then the sample complexity is significantly reduced, to $\tilde O(1 / \varepsilon^2)$, which does not depend on $n$. Our results can be generalized to non-binary events. The proof of our results uses a reduction from the distribution learning problem and reveals the fact that forecast aggregation is almost as difficult as distribution learning.

==> intro_v1.tex <==
\section{Introduction} 
Suppose you want to know whether it will rain tomorrow.  You searched ``weather'' on Google, and it said that the probability of raining was 40\%.  But the weather forecasting app on your phone said 85\%.  And one of your friends, who is an expert in meteorology, said 65\%.  How do you aggregate those multiple predictions into a single one?  
This question is called \emph{forecast aggregation}, or \emph{forecast combination}, in the literature of economic forecasting (e.g., \cite{bates_combination_1969, clemen_combining_1989, timmermann_chapter_2006}). 
It has innumerable applications, ranging from the fields of economics, statistics, operations research, to machine learning, decision theory, and of course, climate science. 

% A known phenomenon in many empirical works on forecast aggregation is the ``forecast combination puzzle'' \cite[p.428]{stock_combination_2004}: a simple aggregation methods like the unweighted averaging of all experts' forecasts often outperform more sophisticated, data-driven, aggregation methods. 

A straightforward solution to the forecast aggregation problem is to simply take the average of all experts' forecasts.
This method does not take into account, for example, the facts that different experts may have different expertise and that their forecasts can be correlated. 
% This method does not take into the underlying information structure governing the experts' predictions and the event being predicted. 
Simple as it is, the averaging method performs surprisingly well in practice, as observed by many forecast aggregation works from 1960s to 2020s (e.g., \cite{bates_combination_1969, newbold_experience_1974, makridakis_averages_1983, gupta_combination_1987, clemen_combining_1989, timmermann_chapter_2006, makridakis_m4_2020}).

One might wonder whether more sophisticated aggregation methods can do better than the simple average.  In particular, a standard approach to forecast aggregation in the literature is the data-driven approach (See Related Works for details).  In some forecasting tasks, we may have historical data of experts' forecasts and the realizations of the predicted events, and using these data we can learn an aggregator via statistics or machine learning techniques. 
For example, we can use a weighted average where the weights of experts are determined by their individual accuracy and correlation estimated from past data. 
Can such methods outperform the simple average? 
% This data-driven approach was proposed even in the first paper on forecast aggregation (Bates and Granger (1969) \cite{bates_combination_1969}) and followed by many works cited above. 

Interestingly, though, the answer is often ``no''.  When researchers tried various data-driven aggregation methods, many of them actually performed \emph{worse} than the simple average (e.g., \cite{makridakis_averages_1983, winkler_combination_1983, gupta_combination_1987, stock_combination_2004, genre_combining_2013}). 
% On the other hand, once researchers turn to more sophisticated, in particular data-driven, aggregation methods, the aggregation performance often \emph{worsen} \cite{makridakis_averages_1983, gupta_combination_1987, stock_combination_2004}.  For example, a weighted average where the weights of experts are determined by their individual prediction accuracy and correlation estimated from past data could perform worse than the simple unweighted average \cite{makridakis_averages_1983}. 
For instance, while weighted averaging methods with weights determined by experts' empirical individual accuracy are sometimes better than the simple average, those incorporating the correlation between experts are usually worse \cite{winkler_combination_1983}. 
The dominance of simple average over sophisticated data-driven methods appeared so many times in practice that it has been known as ``the forecast combination puzzle'' in the literature \cite[p.428]{stock_combination_2004}.
Several explanations to this phenomenon have been given, and the most popular one is, unsurprisingly, \emph{overfitting} \cite{smith_simple_2009, genre_combining_2013, claeskens_forecast_2016}.
Sophisticated data-driven methods usually have many parameters, requiring a large amount of data to estimate, but the sample sizes of many empirical works on forecast aggregation are rather small (24 in \cite{granger_improved_1984}, 69 in \cite{satopaa_combining_2014}, 87 in \cite{baron_two_2014}, 100 in \cite{gupta_combination_1987}).
Too few samples are likely to account for the poor performance of many data-driven methods.

% As noted by, e.g., \cite{gupta_combination_1987, yang_combining_2004, timmermann_chapter_2006}, a possible reason for this is \emph{overfitting}: the amount of data in practice is insufficient for us to find a good aggregation method from a large class of methods: 
% \begin{quote}
%     \emph{While these data-based methods (Minimum Variance and Regression) possess some desirable variance properties, their empirical performance has been disappointing.  ...  This disturbing result likely stems from the large data requirements of those methods. ...  For nonrepetitive events, or nonstationary error generating processes, such large amounts of data may not be available.  In such cases, relying on past data could produce highly erroneous estimates.}
    
%     \hfill --- Gupta and Wilton (1987) \cite[p.358]{gupta_combination_1987}
% \end{quote}

Admittedly, large amounts of samples are indeed difficult to obtain when, e.g., the forecasting tasks are not repetitive and human experts are involved.  However, in many real-world scenarios we do have access to large amounts of samples, at least in principle.  Weather forecast is one such example, where we can collect the forecasts made by algorithms on different days at different locations.  Online forecasting competition platforms like Kaggle also generate huge amounts of data.\footnote{\url{https://www.kaggle.com/c/m5-forecasting-accuracy}}  In those scenarios, it is unclear whether the forecast combination puzzle still persists, or in other words, \emph{how many} samples are needed for a sophisticated data-driven aggregation method to outperform the simple average?
This question motivates our work.  In fact, given that neither the unweighted average nor a weighted average is necessarily the \emph{optimal} aggregation method, we take a step further to ask the following question:
\begin{center}
    \emph{How many samples do we need to achieve optimal aggregation?}
\end{center} 
% 
% Even when we do not have a large amount of samples, our understanding of the forecast combination puzzle is still largely empirical.  Few works have theoretically answered the following question: how many samples do we need to outperform the simple averaging? 
% 
Using terminologies from statistical learning theory \cite{vapnik_nature_2000}, we call this problem ``the sample complexity of forecast aggregation''.

\paragraph{Our contributions}
We initiate the study of sample complexity in forecast aggregation. 
Our first result shows that the sample complexity of forecast aggregation can be extremely large in the worst case.  Specifically, we consider a standard Bayesian forecast model (first developed by \cite{morris_decision_1974, winkler_combining_1981}, surveyed in \cite{geweke_chapter_2006}) as follows: there are $n$ experts, one principal; each expert $i$ observes a private signal $s_i \in \S_i$ that is correlated with an unknown binary event (state of the world) $\omega\in\{0, 1\}$ according to some underlying distribution $P$; experts report their posterior beliefs $r_i = P(\omega = 1 \mid s_i)$ about $\omega$ to the principal, who then aggregates the reports $r_1, \ldots, r_n$ into a single number.
We assume that the principal does not know $P$ but has i.i.d.~samples of experts' reports and event realizations from $P$, based on which it wants to find an aggregator $\hat f: [0, 1]^n \to [0, 1]$ that is ``$\eps$-close'' to the ``optimal'' aggregator $f^*$ (we discuss ``optimality'' in details in Section~\ref{sec:model}), which is the Bayesian aggregator $f^*(r_1, \ldots, r_n) = P(\omega = 1\mid r_1, \ldots, r_n)$, where ``$\eps$-closeness'' is measured in the mean squared difference: $\E_P\big[|\hat f(r_1, \ldots, r_n) - f^*(r_1, \ldots, r_n)|^2\big]\le \eps$. 
Assuming a finite signal space of size $|\S_i| = m$ for each expert, we show that: 
\begin{itemize}
    \item To find an aggregator $\hat f$ that is $\eps$-close to the optimal aggregator $f^*$ with high probability for any distribution $P$, at most $\tilde O(\frac{m^{n}}{\eps^2})$ samples are sufficient, and at least $\tilde \Omega(\frac{m^{n-2}}{\eps})$ samples are necessary\footnote{The $\tilde O(\cdot)$ and $\tilde \Omega(\cdot)$ notations omit logarithmic factors.}. (Theorem~\ref{thm:general_distribution_both}).
\end{itemize}
% This exponential number of samples is never practical, thus supporting the forecast combination puzzle that empirically learned aggregators could be outperformed by a simple averaging in practice.  We also provide an $O(\frac{m^n}{\eps^2})$ sample complexity upper bound (Theorem~\ref{thm:general_distribution_upper_bound}).  Both the lower bound and the upper bound hold for general distribution $P$. 

The exponential sample complexity lower bound $\tilde \Omega(\frac{m^{n-2}}{\eps})$ means that the optimal aggregator $f^*$ is rather difficult to learn, and significantly more difficult when the number of experts increases.  As we show in the proof (which is a reduction from the \emph{distribution learning} problem), this difficulty stems from the fact that we need to estimate the correlation between experts, which requires a large number of samples.
This motivates us to study the special case where (the signals of) experts are conditionally independent, namely, $s_i$'s are independent conditioning on $\omega$. 
The sample complexity is significantly reduced in this case:
\begin{itemize}
    \item If experts are conditionally independent, then an $\eps$-optimal aggregator $\hat f$ can be found with high probability using only $\tilde O(\frac{n}{\eps^2})$ samples.  $\tilde \Omega(\frac{1}{\eps})$ samples are necessary. (Theorem~\ref{thm:conditionally_independent_general}.)
\end{itemize}
The sample complexity upper bound $\tilde O(\frac{n}{\eps^2})$ is linear in $n$ and independent of the signal space size $m$.  
We then further investigate two special conditionally independent cases where the experts are either ``very informative'' or ``very non-informative''.  Under these two special cases, the sample complexity can be $\tilde O(\frac{1}{\eps})$ or even smaller (Theorem~\ref{thm:strongly-informative-upper-bound} and Theorem~\ref{thm:weakly-informative-upper-bound:new}). 


% The significant gap between the sample complexity for general distributions and conditionally independent distributions suggests another form of ``forecast combination puzzle'': aggregation methods that ignore the correlation between experts could perform better than those that take the correlation into account, given a practical sample size.  This phenomenon has actually been observed by empirical works on forecast aggregation \cite{makridakis_averages_1983, gupta_combination_1987, stock_combination_2004}.  Our results hence provide a quantitative theoretical explanation to this phenomenon. 

We review related works in Section~\ref{sec:related_works}.  Section~\ref{sec:model} introduces model and preliminary. 
Section~\ref{sec:general_distribution} studies the sample complexity for general distributions.  Section~\ref{sec:conditionally_independent} considers the conditionally independent case.  Section~\ref{sec:conclusion} concludes and discusses future directions. 

% \paragraph{Structure of the paper}
% We review related works next.  Models and preliminaries are in Section~\ref{sec:model}.  

% \subsection{Overview of Our Results}
% \paragraph{Model} 
% To formalize the sample complexity question above, we consider the following forecast aggregation model, which is a Bayesian framework proposed by Morris (1974) \cite{morris_decision_1974} and more recently studied by \cite{arieli_robust_2018, babichenko_learning_2021, neyman_are_2021}: A principal wants to predict the unknown state of the world $\omega \in \{0, 1\}$.  There are $n$ experts, each observing a private signal $s_i \in \S_i$ that correlates with the state of the world according to some underlying distribution $P$.  Experts know (their marginals of) the distribution $P$ and report their posterior beliefs about $\omega$ to the principal: $r_i = P(\omega = 1 \mid s_i)$.  Given the reports $\bm r = (r_1, \ldots, r_n)$, the principal aggregates them into a single prediction $f(r_1, \ldots, r_n) \in [0, 1]$.  Crucially, we assume that the distribution $P$ is unknown to the principal and can be arbitrarily chosen.  If the principal knows $P$, then it can aggregate ``optimally'' (we formally define ``optimality'' in Section~\ref{sec:model}) using the Bayes' rule: compute the posterior probability of $\omega = 1$ given all the information it receives, $f^*(r_1, \ldots, r_n) = P(\omega = 1 \mid r_1, \ldots, r_n)$.

% The principal has access to $T$ i.i.d.~samples of reports and the realization of the state of the world according to $P$: 
% \begin{equation*}
%     (\bm r^{(1)}, \omega^{(1)}), (\bm r^{(2)}, \omega^{(2)}), ~ \ldots, ~ (\bm r^{(T)}, \omega^{(T)}),  \quad \quad \bm r^{(t)} = (r_1^{(t)}, \ldots, r_n^{(t)}),  
% \end{equation*}
% using which it finds an aggregator $\hat f: [0, 1]^n \to [0, 1]$. 
% An aggregator is $\eps$-optimal if its mean squared difference with $f^*$ is less than $\eps$, where the mean is with respect to $P$: $\E_P\big[|f(\bm r) - f^*(\bm r)|^2\big]\le \eps$. 
% Now, the sample complexity question can be rephrased as follows: 
% \begin{center}
% \emph{How many samples are necessary and sufficient for finding an $\eps$-optimal aggregator \\
% (with high probability over the random draw of samples)?} 
% \end{center}

% \paragraph{Results}
% Unlike many forecast aggregation works that restrict attentions to linear aggregators $\hat f(\bm r) = \sum_{i=1}^n a_i r_i$, we do not put such restrictions on $\hat f$, because we want to approximate the optimal aggregator $f^*$ which need not be linear.  However, such approximation cannot be done with a finite number of samples if $P$ can be an arbitrary continuous distribution.  Hence, our work makes two types of assumptions on $P$: (1) \emph{discrete signal space}: each $\S_i$ is a finite set of size $m < \infty$; (2) \emph{conditionally independent signals}: $s_1, \ldots, s_n$ are independently distributed conditioning on $\omega$.  We prove that, under these assumptions, an $\eps$-optimal aggregator can be found with a finite number of samples.  Specifically, the number of samples is upper bounded by: 
% \begin{itemize}
%     \item Discrete signal space: $O\big(\frac{m^n}{\eps^2}\big)$ (Theorem~\ref{thm:general_distribution_upper_bound}). 
%     \item Conditionally independent signals: $O\big(\frac{(n-1)^2}{\rho \eps}\big)$, where $\rho = \frac{P(\omega = 1)}{P(\omega = 0)}$ is a constant (Theorem~\ref{thm:conditionally_independent_upper_bound}). 
% \end{itemize}

% The above two results answer the ``sufficient'' part in the question we raised above.  The more interesting, and more challenging, part is how many samples are ``necessary''?  We show that, in order to obtain $\eps$-optimal aggregators with high probability, one needs at least the following numbers of samples: 
% \begin{itemize}
%     \item Discrete signal space: $\Omega\big(\frac{m^{n-2}}{\eps}\big)$ (Theorem~\ref{thm:general_distribution_lower_bound}). 
%     \item Conditionally independent signals: $\Omega\big(\frac{1}{\eps}\big)$ (Theorem~\ref{thm:conditionally_independent_lower_bound}). 
% \end{itemize}

% \paragraph{Discussion}
% The exponential sample complexity of learning $\eps$-optimal aggregators for distributions over discrete signal space basically means that learning the optimal aggregator is rather difficult.  As we show in the proof, this difficulty stems from the fact that we need to estimate the correlations between experts.  To estimate such correlations with ``$\eps$-accuracy'', we need $\Omega\big(\frac{m^{n-2}}{\eps}\big)$ samples.
% In practice, this number of samples can hardly be obtained.

% However, once we assume that experts are conditionally independent, the sample complexity significantly reduces.  This could suggest another form of ``forecast combination puzzle'': aggregation methods that ignore the correlations between experts could perform better than those take into account correlations, given a practical number of samples.  This phenomenon has been observed by empirical works \cite{makridakis_averages_1983, gupta_combination_1987, stock_combination_2004}.  Our results provide a rigorous theoretical explanation to this phenomenon. 


% % ===================================================

% % The role of \emph{prior} is important in the forecast aggregation problem. 
% % If we do not have any prior knowledge about the weather or the experts' predicting abilities, then the best we could do is basically some trivial aggregation methods, like taking the average of the experts' predictions, or simply guessing a constant $0.5$.\cite{arieli_robust_2018}. 
% % A natural approach, and in fact a standard approach to the forecast aggregation problem in the literature, is the data-driven approach. 
% % The idea is simple.  

 
% % In practice, we hardly have access to an accurate prior. 
% % A standard approach in the forecast aggregation literature to overcoming this issue is the data-driven approach. 
% % The idea is simple: since many forecasting tasks are repeated (like the weather forecasting example above), we can collect samples of experts' predictions and the outcomes of the predicted event, and use those samples to find a good aggregation method accordingly.  For example, one can use a weighted average where each expert's weight is determined by historical data.

% % This data-driven approach has in fact been a standard approach in the forecast aggregation literature, with numerous empirical works studying how well different aggregation methods work in different real-world forecasting tasks.  See Section~\ref{sec:related_works} for discussions.



% % However, in reality, especially in the weather forecasting example above, the forecasting task is repeated every day, and the outcome of the event being predicted is observed (rain or not).  So, one can observe the historical forecasting performance of each expert and adjust the aggregation method accordingly.  For example, one can use a weighted average aggregation method where each expert's weight is determined by empirical data of its performance.  This data-driven approach has in fact been a standard approach in the forecast aggregation literature, with numerous empirical works studying how well different aggregation methods work in different real-world forecasting tasks.  See Section~\ref{sec:related_works} for discussions.

\subsection{Related Works}\label{sec:related_works}

\paragraph{Data-driven aggregation}
Data-driven approaches to forecast aggregation already appeared in perhaps the first paper on forecast aggregation, Bates and Granger (1969) \cite{bates_combination_1969}, and have been standard in the literature (see surveys \cite{clemen_combining_1989} and \cite{timmermann_chapter_2006}). 
More recent works on data-driven aggregation include, e.g., \cite{satopaa_combining_2014, babichenko_learning_2021, wang_forecast_2021, neyman2022no}.  
Many of these works focus on specific weighted average aggregators like \emph{linear pooling} (weighted arithmetic mean) and \emph{logarithmic pooling} (normalized weighted geometric mean) \cite{satopaa_combining_2014, neyman2022no}, and the goal is to estimate the optimal weights from data, which can be solved by standard statistical tools usually.  
However, those weighted average aggregators are not the optimal \emph{Bayesian} aggregator unless the underlying distribution $P$ of signals and event satisfies some special properties (e.g., experts' forecasts are equal to the true probability of the event plus normally distributed noises \cite{winkler_combining_1981}).  For some distributions the performance of the Bayesian aggregator can be much better than the optimal weighted average. 
Our work aims to understand the sample complexity of Bayesian aggregation, namely how many samples are needed to approximate the Bayesian aggregator.  We think this is a fundamental question that should be addressed.


Our work is closely related to a recent work \cite{babichenko_learning_2021} on Bayesian aggregation via \emph{online learning}.  Assuming conditionally independent experts, \cite{babichenko_learning_2021} shows that one can approximate the Bayesian aggregator with $\eps = \tilde O(n\sqrt T)$ regret.  By an online-to-batch conversion (e.g., \cite{shalev-shwartz_online_2012}, Corollary 5.2), this regret bound implies a $T = \tilde O(\frac{n^2}{\eps^2})$ sample complexity upper bound in the batch learning setting.  We study the batch learning setting directly and obtain an improved bound of $\tilde O(\frac{n}{\eps^2})$.   
However, the loss function considered by \cite{babichenko_learning_2021} is different from ours: theirs is the logarithmic loss while ours is the squared loss.  Since the logarithmic loss is larger than the squared loss, their sample complexity bound should be greater than or equal to our bound.  We do not know whether there is a gap between the tight sample complexity bounds for the two loss functions. 


% \paragraph{Data-driven approaches to forecast aggregation and linear aggregation}
% Data-driven approaches to forecast aggregation already appeared in perhaps the first paper on forecast aggregation, \citet{bates_combination_1969}, and have been a standard practice in forecast aggregation (see, e.g., surveys by \citet{clemen_combining_1989} and \citet{timmermann_chapter_2006}). 
% Many of these works focus on weighted averaging, or more generally \emph{linear} aggregators, $f^{\bm \theta}(r_1, \ldots, r_n) = \sum_{i=1}^n \theta_i r_i + \theta_0$, studying how to use samples to estimate the best coefficient $\bm \theta$. 
% The use of linear aggregators is justified by the fact that the Bayesian optimal aggregator is indeed a linear function when the underlying distribution of experts' forecasts and the event satisfies some conditions, e.g., when experts' forecasts are the true probability of the event plus normally distributed noises (\citet{winkler_combining_1981}).
% While the restriction to linear aggregators and the assumption of normally distributed noise usually suffice for practical purposes, they do not necessarily capture the real underlying relationship between the event and the experts' forecasts.
% The Bayesian optimal aggregator is not linear in general, even for conditionally independent distributions (Section \ref{sec:conditionally_independent}).  
% Our work wants to understand how many samples are needed to approximately identify the Bayesian optimal aggregator.  We think this is a theoretically interesting and important question.
% Another reason why we do not restrict attentions to linear aggregators is that, once restricting to them, the aggregator learning problem reduces to a linear regression, and the sample complexity of aggregation becomes the sample complexity of linear regression, which is conceptually different from our purpose of understanding the sample complexity of aggregation \emph{itself}.
% While the sample complexity of linear aggregation has been studied by \citet{yang_combining_2004}, the sample complexity of Bayesian aggregation has not, as far as we know. 



\paragraph{Robust forecast aggregation}
Some recent works study the 
%There are also works on Bayesian aggregation that are not from a data-driven perspective
Bayesian aggregation problem \emph{not} from a data-driven perspective
\cite{frongillo_elicitation_2015, arieli_robust_2018, neyman_are_2021}.
In particular, \cite{arieli_robust_2018} and \cite{neyman_are_2021} study a ``robust forecast aggregation'' problem where the principal does not know and does not have samples from the prior distribution over experts' forecasts and the event.  They study the worst-case approximation ratio obtainable by a prior-free aggregator compared to the prior-aware Bayesian aggregator.  They give several negative results.  We are able to give positive results ($\eps$-approximation) because of two reasons: (1) we have sample access to the prior; (2) the Bayesian aggregator benchmark they choose is in fact stronger than ours; see Section~\ref{sec:model} for a detailed discussion. 

% problem  (e.g., \cite{arieli_robust_2018, babichenko_learning_2021, neyman_are_2021}) than the traditional forecasting literature (e.g., \cite{bates_combination_1969, morris_combining_1977, winkler_combination_1983, clemen_combining_1989, timmermann_chapter_2006}).
% The latter works usually assume a parametric family of distributions over the the ground truth and the experts' predictions.  Then, the learning task boils down to the estimation of parameters using historical data.

% Non-Bayesian approach: \cite{bates_combination_1969, newbold_experience_1974, winkler_combination_1983, granger_improved_1984}.
% Survey: \cite{clemen_combining_1989, timmermann_chapter_2006}. 

% \paragraph{No-regret learning}
% (e.g., \cite{cesa-bianchi_prediction_2006, frongillo_efficient_2021}) 

% Aggregating forecasts is different from aggregating signals \cite[p.198-199]{granger_improved_1984} \cite[p.168-169]{granger_invited_1989}, \cite[p.143]{timmermann_chapter_2006}. 

% Works about \emph{recalibration} (e.g., \cite{turner_forecast_2014, budescu_identifying_2015}) also study how to choose aggregators based on experts' historical performance.  But those works are mainly empirical: they evaluate the performance of specific aggregator-choosing schemes based on real-world data, without sample complexity analysis.  

\paragraph{Sample complexity of mechanism design}  Our work may remind the reader of a long line of research on the sample complexity of mechanism design, in particular revenue maximization (e.g., \cite{cole_sample_2014, dhangwatnotai_revenue_2015, morgenstern_pseudo-dimension_2015, devanur_sample_2016, balcan_sample_2016, cai_learning_2017, guo_settling_2019, brustle_multi-item_2020, gonczarowski_sample_2021, guo_generalizing_2021}).  A key observation from these works is that, the number of samples needed to learn an $\eps$-optimal auction for $n\ge 1$ independent bidders is increasing in $n$, because when there are more bidders, although we can obtain higher revenue, the optimal auction benchmark also gets improved.  We see a similar phenomenon in the forecast aggregation problem where the sample complexity increases with the number of experts in the general case, but we do not know whether this phenomenon persists when experts are conditionally independent. 


\newpage 


==> intro_v2.tex <==
\section{Introduction} 
Suppose you want to know whether it will rain tomorrow.  You searched ``weather'' on Google, and it said that the probability of raining was 40\%.  But the weather forecasting app on your phone said 85\%.  And one of your friends, who is an expert in meteorology, said 65\%.  How do you aggregate those multiple predictions into a single one?  
This question is called \emph{forecast aggregation}, or \emph{forecast combination}, in the literature of economic forecasting (e.g., \cite{bates_combination_1969, clemen_combining_1989, timmermann_chapter_2006}). 
It has innumerable applications, ranging from the fields of economics, statistics, operations research, to machine learning, decision theory, and of course, climate science. 

A standard approach to forecast aggregation that dates back to the first paper on forecast aggregation in 1969 (Bates and Granger \cite{bates_combination_1969}) is the \emph{data-driven} approach (see, e.g., surveys \cite{clemen_combining_1989, timmermann_chapter_2006} and more recent works \cite{satopaa_combining_2014, babichenko_learning_2021, wang_forecast_2021, neyman2022no}).
Most works on data-driven forecast aggregation focus on the \emph{weighted averaging} aggregation methods.  
The idea is simple: collect experts' predictions in the past, use them to measure each expert's prediction accuracy, and then on a new forecasting task take a weighted average of experts' predictions where a more accurate expert has a larger weight. 
There are different types of weighted averaging and different ways to estimate experts' accuracy.  For example, while the weighted arithmetic mean (aka., \emph{linear pooling}) is a natural choice \cite{bates_combination_1969}, later works advocate the use of normalized weighted geometric mean (aka., \emph{logarithmic pooling}) \cite{genest_aggregating_1984, satopaa_combining_2014, neyman2022no}.
Some works estimate each expert's individual prediction accuracy assuming no correlation among experts, while others argue that correlation should be taken into account  \cite{makridakis_averages_1983, winkler_combination_1983, gupta_combination_1987, stock_combination_2004, genre_combining_2013}.  After a specific weighted averaging method and an accuracy estimation method are chosen, the optimal choice of weights can be found by statistical inference on the historical data (e.g., by linear regression).  

Although weighted averaging methods are popular and perform well in practice (e.g., \cite{bates_combination_1969, newbold_experience_1974, makridakis_averages_1983, gupta_combination_1987, clemen_combining_1989, timmermann_chapter_2006, makridakis_m4_2020}), they are not necessarily the ``best'' way of aggregation.  If one has \emph{prior knowledge} about the experts' prediction process, in the form of a joint distribution over the experts' forecasts and the potential outcome of the predicted event, then the best aggregation method should be the \emph{Bayesian} aggregation \cite{morris_decision_1974, winkler_combining_1981}, namely, use Bayes rule to infer the posterior probability of the event given all experts' forecasts.  Weighted averaging methods are not Bayesian unless the joint distribution over experts' forecasts and the event satisfies some strict assumptions (e.g., experts' forecasts are equal to the true probability of the event plus normally distributed noises \cite{winkler_combining_1981}).  In theory, Bayesian aggregation should perform better (at least not worse) than any weighted averaging.  But in practice this is not always the case, due to reasons like incorrect prior and, in particular, the lack of historical data, especially given the small sample sizes in many empirical works on forecast aggregation (24 in \cite{granger_improved_1984}, 69 in \cite{satopaa_combining_2014}, 87 in \cite{baron_two_2014}, 100 in \cite{gupta_combination_1987}).  

Admittedly, large amounts of data/samples are difficult to obtain when, e.g., the forecasting task is not repetitive and human experts are involved.  But in many modern algorithm-aided forecasting tasks we could potentially obtain large amounts of data.  Weather forecast is one such example, where we can collect the forecasts made by algorithms on different days at different locations.  Online forecasting competition platforms like Kaggle also generate huge amounts of data.\footnote{\url{https://www.kaggle.com/c/m5-forecasting-accuracy}}  In those scenarios, one can actually hope to outperform the simple weighted averaging methods by using more sophisticated data-driven methods, and even implement the optimal method, the Bayesian one, using a large amount of samples.
A natural question then follows: \emph{how many} samples are needed to achieve these goals?   This question motivates our work.


\paragraph{Our contributions}
We initiate the study of \emph{sample complexity of forecast aggregation}, namely: 
\begin{center}
    \emph{How many samples do we need to approximate the optimal (Bayesian) aggregation?}
\end{center} 

Our first result shows that the sample complexity of forecast aggregation can be extremely large in the worst case.  Specifically, we consider a standard Bayesian forecast model as follows: there are $n$ experts, one principal; each expert $i$ observes a private signal $s_i \in \S_i$ that is correlated with an unknown binary event (state of the world) $\omega\in\{0, 1\}$ according to some underlying distribution $P$; experts report their posterior beliefs $r_i = P(\omega = 1 \mid s_i)$ about $\omega$ to the principal, who then aggregates the reports $r_1, \ldots, r_n$ into a single number.
We assume that the principal does not know $P$ but has i.i.d.~samples of experts' reports and event realizations from $P$, based on which it wants to find an aggregator $\hat f: [0, 1]^n \to [0, 1]$ that is ``$\eps$-close'' to the ``optimal'' aggregator $f^*$ (we discuss ``optimality'' in details in Section~\ref{sec:model}), which is the Bayesian aggregator $f^*(r_1, \ldots, r_n) = P(\omega = 1\mid r_1, \ldots, r_n)$, where ``$\eps$-closeness'' is measured in the mean squared difference: $\E_P\big[|\hat f(r_1, \ldots, r_n) - f^*(r_1, \ldots, r_n)|^2\big]\le \eps$. 
Assuming a finite signal space of size $|\S_i| = m$ for each expert, we show that: 
\begin{itemize}
    \item To find an aggregator $\hat f$ that is $\eps$-close to the optimal aggregator $f^*$ with high probability for any distribution $P$, at most $\tilde O(\frac{m^{n}}{\eps^2})$ samples are sufficient, and at least $\tilde \Omega(\frac{m^{n-2}}{\eps})$ samples are necessary\footnote{The $\tilde O(\cdot)$ and $\tilde \Omega(\cdot)$ notations omit logarithmic factors.}. (Theorem~\ref{thm:general_distribution_both}).
\end{itemize}
% This exponential number of samples is never practical, thus supporting the forecast combination puzzle that empirically learned aggregators could be outperformed by a simple averaging in practice.  We also provide an $O(\frac{m^n}{\eps^2})$ sample complexity upper bound (Theorem~\ref{thm:general_distribution_upper_bound}).  Both the lower bound and the upper bound hold for general distribution $P$. 

The exponential sample complexity lower bound $\tilde \Omega(\frac{m^{n-2}}{\eps})$ means that the optimal aggregator $f^*$ is rather difficult to learn, and significantly more difficult when the number of experts increases.  As we show in the proof (which is a reduction from the \emph{distribution learning} problem), this difficulty stems from the fact that we need to estimate the correlation between experts, which requires a large number of samples.
This motivates us to study the special case where (the signals of) experts are conditionally independent, namely, $s_i$'s are independent conditioning on $\omega$. 
The sample complexity is significantly reduced in this case:
\begin{itemize}
    \item If experts are conditionally independent, then an $\eps$-optimal aggregator $\hat f$ can be found with high probability using only $\tilde O(\frac{n}{\eps^2})$ samples.  $\tilde \Omega(\frac{1}{\eps})$ samples are necessary. (Theorem~\ref{thm:conditionally_independent_general}.)
\end{itemize}
The sample complexity upper bound $\tilde O(\frac{n}{\eps^2})$ is linear in $n$ and independent of the signal space size $m$.  
We then further investigate two special conditionally independent cases where the experts are either ``very informative'' or ``very non-informative''.  Under these two special cases, the sample complexity can be $\tilde O(\frac{1}{\eps})$ or even smaller (Theorem~\ref{thm:strongly-informative-upper-bound} and Theorem~\ref{thm:weakly-informative-upper-bound:new}). 


% The significant gap between the sample complexity for general distributions and conditionally independent distributions suggests another form of ``forecast combination puzzle'': aggregation methods that ignore the correlation between experts could perform better than those that take the correlation into account, given a practical sample size.  This phenomenon has actually been observed by empirical works on forecast aggregation \cite{makridakis_averages_1983, gupta_combination_1987, stock_combination_2004}.  Our results hence provide a quantitative theoretical explanation to this phenomenon. 

We review related works in Section~\ref{sec:related_works}.  Section~\ref{sec:model} introduces model and preliminary. 
Section~\ref{sec:general_distribution} studies the sample complexity for general distributions.  Section~\ref{sec:conditionally_independent} considers the conditionally independent case.  Section~\ref{sec:conclusion} concludes and discusses future directions. 

% \paragraph{Structure of the paper}
% We review related works next.  Models and preliminaries are in Section~\ref{sec:model}.  

% \subsection{Overview of Our Results}
% \paragraph{Model} 
% To formalize the sample complexity question above, we consider the following forecast aggregation model, which is a Bayesian framework proposed by Morris (1974) \cite{morris_decision_1974} and more recently studied by \cite{arieli_robust_2018, babichenko_learning_2021, neyman_are_2021}: A principal wants to predict the unknown state of the world $\omega \in \{0, 1\}$.  There are $n$ experts, each observing a private signal $s_i \in \S_i$ that correlates with the state of the world according to some underlying distribution $P$.  Experts know (their marginals of) the distribution $P$ and report their posterior beliefs about $\omega$ to the principal: $r_i = P(\omega = 1 \mid s_i)$.  Given the reports $\bm r = (r_1, \ldots, r_n)$, the principal aggregates them into a single prediction $f(r_1, \ldots, r_n) \in [0, 1]$.  Crucially, we assume that the distribution $P$ is unknown to the principal and can be arbitrarily chosen.  If the principal knows $P$, then it can aggregate ``optimally'' (we formally define ``optimality'' in Section~\ref{sec:model}) using the Bayes' rule: compute the posterior probability of $\omega = 1$ given all the information it receives, $f^*(r_1, \ldots, r_n) = P(\omega = 1 \mid r_1, \ldots, r_n)$.

% The principal has access to $T$ i.i.d.~samples of reports and the realization of the state of the world according to $P$: 
% \begin{equation*}
%     (\bm r^{(1)}, \omega^{(1)}), (\bm r^{(2)}, \omega^{(2)}), ~ \ldots, ~ (\bm r^{(T)}, \omega^{(T)}),  \quad \quad \bm r^{(t)} = (r_1^{(t)}, \ldots, r_n^{(t)}),  
% \end{equation*}
% using which it finds an aggregator $\hat f: [0, 1]^n \to [0, 1]$. 
% An aggregator is $\eps$-optimal if its mean squared difference with $f^*$ is less than $\eps$, where the mean is with respect to $P$: $\E_P\big[|f(\bm r) - f^*(\bm r)|^2\big]\le \eps$. 
% Now, the sample complexity question can be rephrased as follows: 
% \begin{center}
% \emph{How many samples are necessary and sufficient for finding an $\eps$-optimal aggregator \\
% (with high probability over the random draw of samples)?} 
% \end{center}

% \paragraph{Results}
% Unlike many forecast aggregation works that restrict attentions to linear aggregators $\hat f(\bm r) = \sum_{i=1}^n a_i r_i$, we do not put such restrictions on $\hat f$, because we want to approximate the optimal aggregator $f^*$ which need not be linear.  However, such approximation cannot be done with a finite number of samples if $P$ can be an arbitrary continuous distribution.  Hence, our work makes two types of assumptions on $P$: (1) \emph{discrete signal space}: each $\S_i$ is a finite set of size $m < \infty$; (2) \emph{conditionally independent signals}: $s_1, \ldots, s_n$ are independently distributed conditioning on $\omega$.  We prove that, under these assumptions, an $\eps$-optimal aggregator can be found with a finite number of samples.  Specifically, the number of samples is upper bounded by: 
% \begin{itemize}
%     \item Discrete signal space: $O\big(\frac{m^n}{\eps^2}\big)$ (Theorem~\ref{thm:general_distribution_upper_bound}). 
%     \item Conditionally independent signals: $O\big(\frac{(n-1)^2}{\rho \eps}\big)$, where $\rho = \frac{P(\omega = 1)}{P(\omega = 0)}$ is a constant (Theorem~\ref{thm:conditionally_independent_upper_bound}). 
% \end{itemize}

% The above two results answer the ``sufficient'' part in the question we raised above.  The more interesting, and more challenging, part is how many samples are ``necessary''?  We show that, in order to obtain $\eps$-optimal aggregators with high probability, one needs at least the following numbers of samples: 
% \begin{itemize}
%     \item Discrete signal space: $\Omega\big(\frac{m^{n-2}}{\eps}\big)$ (Theorem~\ref{thm:general_distribution_lower_bound}). 
%     \item Conditionally independent signals: $\Omega\big(\frac{1}{\eps}\big)$ (Theorem~\ref{thm:conditionally_independent_lower_bound}). 
% \end{itemize}

% \paragraph{Discussion}
% The exponential sample complexity of learning $\eps$-optimal aggregators for distributions over discrete signal space basically means that learning the optimal aggregator is rather difficult.  As we show in the proof, this difficulty stems from the fact that we need to estimate the correlations between experts.  To estimate such correlations with ``$\eps$-accuracy'', we need $\Omega\big(\frac{m^{n-2}}{\eps}\big)$ samples.
% In practice, this number of samples can hardly be obtained.

% However, once we assume that experts are conditionally independent, the sample complexity significantly reduces.  This could suggest another form of ``forecast combination puzzle'': aggregation methods that ignore the correlations between experts could perform better than those take into account correlations, given a practical number of samples.  This phenomenon has been observed by empirical works \cite{makridakis_averages_1983, gupta_combination_1987, stock_combination_2004}.  Our results provide a rigorous theoretical explanation to this phenomenon. 


% % ===================================================

% % The role of \emph{prior} is important in the forecast aggregation problem. 
% % If we do not have any prior knowledge about the weather or the experts' predicting abilities, then the best we could do is basically some trivial aggregation methods, like taking the average of the experts' predictions, or simply guessing a constant $0.5$.\cite{arieli_robust_2018}. 
% % A natural approach, and in fact a standard approach to the forecast aggregation problem in the literature, is the data-driven approach. 
% % The idea is simple.  

 
% % In practice, we hardly have access to an accurate prior. 
% % A standard approach in the forecast aggregation literature to overcoming this issue is the data-driven approach. 
% % The idea is simple: since many forecasting tasks are repeated (like the weather forecasting example above), we can collect samples of experts' predictions and the outcomes of the predicted event, and use those samples to find a good aggregation method accordingly.  For example, one can use a weighted average where each expert's weight is determined by historical data.

% % This data-driven approach has in fact been a standard approach in the forecast aggregation literature, with numerous empirical works studying how well different aggregation methods work in different real-world forecasting tasks.  See Section~\ref{sec:related_works} for discussions.



% % However, in reality, especially in the weather forecasting example above, the forecasting task is repeated every day, and the outcome of the event being predicted is observed (rain or not).  So, one can observe the historical forecasting performance of each expert and adjust the aggregation method accordingly.  For example, one can use a weighted average aggregation method where each expert's weight is determined by empirical data of its performance.  This data-driven approach has in fact been a standard approach in the forecast aggregation literature, with numerous empirical works studying how well different aggregation methods work in different real-world forecasting tasks.  See Section~\ref{sec:related_works} for discussions.

\subsection{Related Works}\label{sec:related_works}


\paragraph{Data-driven aggregation}
Since the seminal work of Bates and Granger (1969) \cite{bates_combination_1969}, many researchers have tried various data-driven methods for the forecast aggregation problem, including weighted averaging, \tl{give more examples here}, and neural network based aggregators (e.g., \cite{makridakis_averages_1983, winkler_combination_1983, gupta_combination_1987, stock_combination_2004, genre_combining_2013}). 
A common phenomenon found in these works is  ``the forecast combination puzzle'' \cite[p.428]{stock_combination_2004}: sophisticated data-driven methods often perform \emph{worse} than simple ones. 
For example, a weighted averaging method where the weights of experts are determined by both their individual accuracy and correlation estimated from past data can be worse than the method that considers individual accuracy only, ignoring correlation \cite{winkler_combination_1983}.  
Explanations to the forecast combination puzzle have been given, and the most popular one is, unsurprisingly, \emph{overfitting} \cite{smith_simple_2009, genre_combining_2013, claeskens_forecast_2016}.
Optimizing a sophisticated data-driven method requires a large amount of data, but data are few in practice.
We therefore think that it is an important question, from both theoretical and practical points of view, to understand exactly how many samples are needed to learn a better aggregator than a simple one like the averaging.  In this work, we focus on the optimal aggregator, the Bayesian aggregator, specifically.
%  We study the sample complexity of Bayesian aggregation, namely how many samples are needed to approximate the Bayesian aggregator.
% We think the sample complexity of Bayesian aggregation is a fundamental question that should be addressed.


Our work is closely related to a recent work \cite{babichenko_learning_2021} on Bayesian aggregation via \emph{online learning}.  Assuming conditionally independent experts, \cite{babichenko_learning_2021} shows that one can approximate the Bayesian aggregator with $\eps = \tilde O(n\sqrt T)$ regret.  By an online-to-batch conversion (e.g., \cite{shalev-shwartz_online_2012}, Corollary 5.2), this regret bound implies a $T = \tilde O(\frac{n^2}{\eps^2})$ sample complexity upper bound in the batch learning setting.  We study the batch learning setting directly and obtain an improved bound of $\tilde O(\frac{n}{\eps^2})$.   
However, the loss function considered by \cite{babichenko_learning_2021} is different from ours: theirs is the logarithmic loss while ours is the squared loss.  Since the logarithmic loss is larger than the squared loss, their sample complexity bound should be greater than or equal to our bound.  We do not know whether there is a gap between the tight sample complexity bounds for the two loss functions. 


% \paragraph{Data-driven approaches to forecast aggregation and linear aggregation}
% Data-driven approaches to forecast aggregation already appeared in perhaps the first paper on forecast aggregation, \citet{bates_combination_1969}, and have been a standard practice in forecast aggregation (see, e.g., surveys by \citet{clemen_combining_1989} and \citet{timmermann_chapter_2006}). 
% Many of these works focus on weighted averaging, or more generally \emph{linear} aggregators, $f^{\bm \theta}(r_1, \ldots, r_n) = \sum_{i=1}^n \theta_i r_i + \theta_0$, studying how to use samples to estimate the best coefficient $\bm \theta$. 
% The use of linear aggregators is justified by the fact that the Bayesian optimal aggregator is indeed a linear function when the underlying distribution of experts' forecasts and the event satisfies some conditions, e.g., when experts' forecasts are the true probability of the event plus normally distributed noises (\citet{winkler_combining_1981}).
% While the restriction to linear aggregators and the assumption of normally distributed noise usually suffice for practical purposes, they do not necessarily capture the real underlying relationship between the event and the experts' forecasts.
% The Bayesian optimal aggregator is not linear in general, even for conditionally independent distributions (Section \ref{sec:conditionally_independent}).  
% Our work wants to understand how many samples are needed to approximately identify the Bayesian optimal aggregator.  We think this is a theoretically interesting and important question.
% Another reason why we do not restrict attentions to linear aggregators is that, once restricting to them, the aggregator learning problem reduces to a linear regression, and the sample complexity of aggregation becomes the sample complexity of linear regression, which is conceptually different from our purpose of understanding the sample complexity of aggregation \emph{itself}.
% While the sample complexity of linear aggregation has been studied by \citet{yang_combining_2004}, the sample complexity of Bayesian aggregation has not, as far as we know. 


\paragraph{Robust forecast aggregation}
Some recent works study the 
%There are also works on Bayesian aggregation that are not from a data-driven perspective
Bayesian aggregation problem \emph{not} from a data-driven perspective
\cite{frongillo_elicitation_2015, arieli_robust_2018, neyman_are_2021}.
In particular, \cite{arieli_robust_2018} and \cite{neyman_are_2021} study a ``robust forecast aggregation'' problem where the principal does not know and does not have samples from the prior distribution over experts' forecasts and the event.  They study the worst-case approximation ratio obtainable by a prior-free aggregator compared to the prior-aware Bayesian aggregator.  They give several negative results.  We are able to give positive results ($\eps$-approximation) because of two reasons: (1) we have sample access to the prior; (2) the Bayesian aggregator benchmark they choose is in fact stronger than ours; see Section~\ref{sec:model} for a detailed discussion. 

% problem  (e.g., \cite{arieli_robust_2018, babichenko_learning_2021, neyman_are_2021}) than the traditional forecasting literature (e.g., \cite{bates_combination_1969, morris_combining_1977, winkler_combination_1983, clemen_combining_1989, timmermann_chapter_2006}).
% The latter works usually assume a parametric family of distributions over the the ground truth and the experts' predictions.  Then, the learning task boils down to the estimation of parameters using historical data.

% Non-Bayesian approach: \cite{bates_combination_1969, newbold_experience_1974, winkler_combination_1983, granger_improved_1984}.
% Survey: \cite{clemen_combining_1989, timmermann_chapter_2006}. 

% \paragraph{No-regret learning}
% (e.g., \cite{cesa-bianchi_prediction_2006, frongillo_efficient_2021}) 

% Aggregating forecasts is different from aggregating signals \cite[p.198-199]{granger_improved_1984} \cite[p.168-169]{granger_invited_1989}, \cite[p.143]{timmermann_chapter_2006}. 

% Works about \emph{recalibration} (e.g., \cite{turner_forecast_2014, budescu_identifying_2015}) also study how to choose aggregators based on experts' historical performance.  But those works are mainly empirical: they evaluate the performance of specific aggregator-choosing schemes based on real-world data, without sample complexity analysis.  

\paragraph{Sample complexity of mechanism design}  Our work may remind the reader of a long line of research on the sample complexity of mechanism design, in particular revenue maximization (e.g., \cite{cole_sample_2014, dhangwatnotai_revenue_2015, morgenstern_pseudo-dimension_2015, devanur_sample_2016, balcan_sample_2016, cai_learning_2017, guo_settling_2019, brustle_multi-item_2020, gonczarowski_sample_2021, guo_generalizing_2021}).  A key observation from these works is that, the number of samples needed to learn an $\eps$-optimal auction for $n\ge 1$ independent bidders is increasing in $n$, because when there are more bidders, although we can obtain higher revenue, the optimal auction benchmark also gets improved.  We see a similar phenomenon in the forecast aggregation problem where the sample complexity increases with the number of experts in the general case, but we do not know whether this phenomenon persists when experts are conditionally independent. 


==> intro_v3.tex <==
\section{Introduction} 
Suppose you want to know whether it will rain tomorrow.  You search ``weather'' on Google, and it says that the probability of raining tomorrow is 40\%.  But the weather forecasting app on your phone shows 85\%.  And one of your friends, who is an expert in meteorology, predicts 65\%.  How do you aggregate these predictions into a single one?  
This problem is called \emph{forecast aggregation} or \emph{forecast combination} (e.g., \cite{bates_combination_1969, clemen_combining_1989, timmermann_chapter_2006}).
\yc{Is this literature is really called economic forecasting? The cited papers were not published in the econ journals.}
\tl{I deleted the word ``economic forecasting''}
It has innumerable applications in fields ranging from economics, statistics, operations research, to machine learning, decision theory, and of course, climate science. 

% A known phenomenon in many empirical works on forecast aggregation is the ``forecast combination puzzle'' \cite[p.428]{stock_combination_2004}: a simple aggregation methods like the unweighted averaging of all experts' forecasts often outperform more sophisticated, data-driven, aggregation methods. 

A straightforward solution to the forecast aggregation problem is to simply take the (unweighted) average of all experts' forecasts.
This does not take into account, for example, the fact that different experts may have different expertise. 
Simple as it is, this method performs surprisingly well in practice, as observed by many forecast aggregation works from 1960s to 2020s (e.g., \cite{bates_combination_1969, newbold_experience_1974, makridakis_averages_1983, gupta_combination_1987, clemen_combining_1989, timmermann_chapter_2006, makridakis_m4_2020}).

Naturally, one can think of more sophisticated aggregation methods than the simple averaging.  In particular, since many forecasting tasks in practice are repetitive, like weather forecast, one can actually use \emph{data-driven} aggregation methods:  
%, which in fact is a standard approach to forecast aggregation that dates back to perhaps the first paper on forecast aggregation (Bates and Granger, 1969, \cite{bates_combination_1969}).
first collect experts' forecasts and the realizations of the predicted events in the past, then use those data to learn an aggregator for future forecasting tasks. 
For example, one can use a weighted average where the weights of experts are determined by their historical prediction accuracy, or train a neural network aggregator from data.
Can such data-driven methods outperform the simple unweighted average? 
% This data-driven approach was proposed even in the first paper on forecast aggregation (Bates and Granger (1969) \cite{bates_combination_1969}) and followed by many works cited above. 

Interestingly, though, the answer is often ``no''.  When researchers try various data-driven aggregation methods, many of them actually perform \emph{worse} than the simple average (e.g., \cite{makridakis_averages_1983, winkler_combination_1983, gupta_combination_1987, stock_combination_2004, genre_combining_2013}). 
% On the other hand, once researchers turn to more sophisticated, in particular data-driven, aggregation methods, the aggregation performance often \emph{worsen} \cite{makridakis_averages_1983, gupta_combination_1987, stock_combination_2004}.  For example, a weighted average where the weights of experts are determined by their individual prediction accuracy and correlation estimated from past data could perform worse than the simple unweighted average \cite{makridakis_averages_1983}. 
For instance, while weighted averaging methods with weights determined by experts' individual accuracy are sometimes better than the simple average, those taking into account the correlations between experts are usually worse \cite{winkler_combination_1983}. 
The dominance of simple average over sophisticated data-driven methods appeared so often in practice that it has been known as ``the forecast combination puzzle'' in the literature \cite[p.428]{stock_combination_2004}.
Several explanations to this puzzle have been given, and a prominent one is, unsurprisingly, \emph{overfitting} \cite{smith_simple_2009, genre_combining_2013, claeskens_forecast_2016}: 
sophisticated data-driven methods require large amounts of data to optimize, but the sample sizes in many empirical forecast aggregation works  are rather small (24 in \cite{granger_improved_1984}, 69 in \cite{satopaa_combining_2014}, 87 in \cite{baron_two_2014}, 100 in \cite{gupta_combination_1987}).
The lack of data is likely to account for the poor performance of many data-driven methods in practice.

% As noted by, e.g., \cite{gupta_combination_1987, yang_combining_2004, timmermann_chapter_2006}, a possible reason for this is \emph{overfitting}: the amount of data in practice is insufficient for us to find a good aggregation method from a large class of methods: 
% \begin{quote}
%     \emph{While these data-based methods (Minimum Variance and Regression) possess some desirable variance properties, their empirical performance has been disappointing.  ...  This disturbing result likely stems from the large data requirements of those methods. ...  For nonrepetitive events, or nonstationary error generating processes, such large amounts of data may not be available.  In such cases, relying on past data could produce highly erroneous estimates.}
    
%     \hfill --- Gupta and Wilton (1987) \cite[p.358]{gupta_combination_1987}
% \end{quote}

Admittedly, data are difficult to obtain when, e.g., the forecasting task is not repetitive and human experts are involved.  However, in many repetitive, algorithm-driven, forecasting tasks we do have abundant data.  Weather forecast is one example, where we have forecasts made by algorithms on different days at different locations.  Online forecasting competition platforms like Kaggle also generate huge amounts of data.\footnote{\url{https://www.kaggle.com/c/m5-forecasting-accuracy}}  In those scenarios, one can actually hope for some data-driven methods to outperform the simple average.  Taking a step further, one might wonder:  What is the \emph{best} aggregation one can hopefully achieve given an infinite amount of data?  How many data/samples are needed to approximately achieve that? 
These questions motivate our work.

% 
% Even when we do not have a large amount of samples, our understanding of the forecast combination puzzle is still largely empirical.  Few works have theoretically answered the following question: how many samples do we need to outperform the simple averaging? 
% 
% Using terminologies from statistical learning theory \cite{vapnik_nature_2000}, we call this problem ``the sample complexity of forecast aggregation''.

\paragraph{Our contributions}
We initiate the study of \emph{sample complexity of forecast aggregation}, namely:  
\begin{center}
    \emph{How many samples do we need to achieve the optimal aggregation approximately?}
\end{center} 

Our first result shows that the sample complexity of forecast aggregation can be extremely large in the worst case.  This partly explains why sophisticated data-driven methods hardly outperform the simple averaging.  Specifically, we consider a standard Bayesian forecast model (first developed by \cite{morris_decision_1974, winkler_combining_1981}, surveyed in \cite{geweke_chapter_2006}) as follows: there are $n$ experts, one principal; each expert $i$ observes a private signal $s_i \in \S_i$ about an unknown binary event (state of the world) $\omega\in\{0, 1\}$; experts' signals and the event jointly follow an underlying distribution $P$; each expert reports their posterior belief $r_i = P(\omega = 1 \,|\, s_i)$ about $\omega$ to the principal, who then aggregates all the reports $r_1, \ldots, r_n$ into a single prediction for $\omega$.
We assume that the principal does not know $P$ but has i.i.d.~samples of experts' reports (not signals) and event realizations from $P$, based on which it wants to find an aggregator $\hat f: [0, 1]^n \to [0, 1]$ that is ``$\eps$-close'' to the ``optimal'' aggregator $f^*$ (we define ``optimal'' in Section~\ref{sec:model}), which is the Bayesian aggregator $f^*(r_1, \ldots, r_n) = P(\omega = 1 \,|\, r_1, \ldots, r_n)$, where ``$\eps$-closeness'' is measured in the mean squared difference: $\E_P\big[|\hat f(r_1, \ldots, r_n) - f^*(r_1, \ldots, r_n)|^2\big]\le \eps$. 
Assuming a finite signal space of size $|\S_i| = m$ for each expert, we show that: 
\begin{itemize}
    \item To find an aggregator $\hat f$ that is $\eps$-close to the optimal aggregator $f^*$ with high probability for any distribution $P$, at most $\tilde O(\frac{m^{n}}{\eps^2})$ samples are sufficient, and at least $\tilde \Omega(\frac{m^{n-2}}{\eps})$ samples are necessary.\footnote{The $\tilde O(\cdot)$ and $\tilde \Omega(\cdot)$ notations omit logarithmic factors.} (Theorem~\ref{thm:general_distribution_both}.)
\end{itemize}
% This exponential number of samples is never practical, thus supporting the forecast combination puzzle that empirically learned aggregators could be outperformed by a simple averaging in practice.  We also provide an $O(\frac{m^n}{\eps^2})$ sample complexity upper bound (Theorem~\ref{thm:general_distribution_upper_bound}).  Both the lower bound and the upper bound hold for general distribution $P$. 

The exponential sample complexity lower bound $\tilde \Omega(\frac{m^{n-2}}{\eps})$ means that the optimal aggregator $f^*$ is rather difficult to learn, and significantly more difficult when the number of experts increases.  As we show in the proof (which is a reduction from the \emph{distribution learning} problem), this difficulty stems from the fact that we need to estimate the correlation between experts, which requires a large number of samples.
This motivates us to study the special case where (the signals of) experts are conditionally independent, namely, $s_i$'s are independent conditioning on $\omega$. 
The sample complexity is significantly reduced in this case:
\begin{itemize}
    \item If experts are conditionally independent, then an $\eps$-optimal aggregator $\hat f$ can be found with high probability using only $\tilde O(\frac{n}{\eps^2})$ samples.  $\tilde \Omega(\frac{1}{\eps})$ samples are necessary. (Theorem~\ref{thm:conditionally_independent_general}.)
\end{itemize}

The sample complexity upper bound $\tilde O(\frac{n}{\eps^2})$ in the conditionally independent case is only linear in $n$ and independent of the signal space size $m$.  
We then further investigate two special conditionally independent cases where the experts are either ``very informative'' or ``very non-informative''.  Under both cases the sample complexity can be $\tilde O(\frac{1}{\eps})$ or even smaller (Theorem~\ref{thm:strongly-informative-upper-bound} and \ref{thm:weakly-informative-upper-bound:new}). 


% The significant gap between the sample complexity for general distributions and conditionally independent distributions suggests another form of ``forecast combination puzzle'': aggregation methods that ignore the correlation between experts could perform better than those that take the correlation into account, given a practical sample size.  This phenomenon has actually been observed by empirical works on forecast aggregation \cite{makridakis_averages_1983, gupta_combination_1987, stock_combination_2004}.  Our results hence provide a quantitative theoretical explanation to this phenomenon. 

We review related works in Section~\ref{sec:related_works}.  Section~\ref{sec:model} introduces model and preliminary. 
Section~\ref{sec:general_distribution} studies the sample complexity for general distributions.  Section~\ref{sec:conditionally_independent} considers the conditionally independent case.  Section~\ref{sec:conclusion} concludes and discusses future directions. 

% \paragraph{Structure of the paper}
% We review related works next.  Models and preliminaries are in Section~\ref{sec:model}.  

% \subsection{Overview of Our Results}
% \paragraph{Model} 
% To formalize the sample complexity question above, we consider the following forecast aggregation model, which is a Bayesian framework proposed by Morris (1974) \cite{morris_decision_1974} and more recently studied by \cite{arieli_robust_2018, babichenko_learning_2021, neyman_are_2021}: A principal wants to predict the unknown state of the world $\omega \in \{0, 1\}$.  There are $n$ experts, each observing a private signal $s_i \in \S_i$ that correlates with the state of the world according to some underlying distribution $P$.  Experts know (their marginals of) the distribution $P$ and report their posterior beliefs about $\omega$ to the principal: $r_i = P(\omega = 1 \mid s_i)$.  Given the reports $\bm r = (r_1, \ldots, r_n)$, the principal aggregates them into a single prediction $f(r_1, \ldots, r_n) \in [0, 1]$.  Crucially, we assume that the distribution $P$ is unknown to the principal and can be arbitrarily chosen.  If the principal knows $P$, then it can aggregate ``optimally'' (we formally define ``optimality'' in Section~\ref{sec:model}) using the Bayes' rule: compute the posterior probability of $\omega = 1$ given all the information it receives, $f^*(r_1, \ldots, r_n) = P(\omega = 1 \mid r_1, \ldots, r_n)$.

% The principal has access to $T$ i.i.d.~samples of reports and the realization of the state of the world according to $P$: 
% \begin{equation*}
%     (\bm r^{(1)}, \omega^{(1)}), (\bm r^{(2)}, \omega^{(2)}), ~ \ldots, ~ (\bm r^{(T)}, \omega^{(T)}),  \quad \quad \bm r^{(t)} = (r_1^{(t)}, \ldots, r_n^{(t)}),  
% \end{equation*}
% using which it finds an aggregator $\hat f: [0, 1]^n \to [0, 1]$. 
% An aggregator is $\eps$-optimal if its mean squared difference with $f^*$ is less than $\eps$, where the mean is with respect to $P$: $\E_P\big[|f(\bm r) - f^*(\bm r)|^2\big]\le \eps$. 
% Now, the sample complexity question can be rephrased as follows: 
% \begin{center}
% \emph{How many samples are necessary and sufficient for finding an $\eps$-optimal aggregator \\
% (with high probability over the random draw of samples)?} 
% \end{center}

% \paragraph{Results}
% Unlike many forecast aggregation works that restrict attentions to linear aggregators $\hat f(\bm r) = \sum_{i=1}^n a_i r_i$, we do not put such restrictions on $\hat f$, because we want to approximate the optimal aggregator $f^*$ which need not be linear.  However, such approximation cannot be done with a finite number of samples if $P$ can be an arbitrary continuous distribution.  Hence, our work makes two types of assumptions on $P$: (1) \emph{discrete signal space}: each $\S_i$ is a finite set of size $m < \infty$; (2) \emph{conditionally independent signals}: $s_1, \ldots, s_n$ are independently distributed conditioning on $\omega$.  We prove that, under these assumptions, an $\eps$-optimal aggregator can be found with a finite number of samples.  Specifically, the number of samples is upper bounded by: 
% \begin{itemize}
%     \item Discrete signal space: $O\big(\frac{m^n}{\eps^2}\big)$ (Theorem~\ref{thm:general_distribution_upper_bound}). 
%     \item Conditionally independent signals: $O\big(\frac{(n-1)^2}{\rho \eps}\big)$, where $\rho = \frac{P(\omega = 1)}{P(\omega = 0)}$ is a constant (Theorem~\ref{thm:conditionally_independent_upper_bound}). 
% \end{itemize}

% The above two results answer the ``sufficient'' part in the question we raised above.  The more interesting, and more challenging, part is how many samples are ``necessary''?  We show that, in order to obtain $\eps$-optimal aggregators with high probability, one needs at least the following numbers of samples: 
% \begin{itemize}
%     \item Discrete signal space: $\Omega\big(\frac{m^{n-2}}{\eps}\big)$ (Theorem~\ref{thm:general_distribution_lower_bound}). 
%     \item Conditionally independent signals: $\Omega\big(\frac{1}{\eps}\big)$ (Theorem~\ref{thm:conditionally_independent_lower_bound}). 
% \end{itemize}

% \paragraph{Discussion}
% The exponential sample complexity of learning $\eps$-optimal aggregators for distributions over discrete signal space basically means that learning the optimal aggregator is rather difficult.  As we show in the proof, this difficulty stems from the fact that we need to estimate the correlations between experts.  To estimate such correlations with ``$\eps$-accuracy'', we need $\Omega\big(\frac{m^{n-2}}{\eps}\big)$ samples.
% In practice, this number of samples can hardly be obtained.

% However, once we assume that experts are conditionally independent, the sample complexity significantly reduces.  This could suggest another form of ``forecast combination puzzle'': aggregation methods that ignore the correlations between experts could perform better than those take into account correlations, given a practical number of samples.  This phenomenon has been observed by empirical works \cite{makridakis_averages_1983, gupta_combination_1987, stock_combination_2004}.  Our results provide a rigorous theoretical explanation to this phenomenon. 


% % ===================================================

% % The role of \emph{prior} is important in the forecast aggregation problem. 
% % If we do not have any prior knowledge about the weather or the experts' predicting abilities, then the best we could do is basically some trivial aggregation methods, like taking the average of the experts' predictions, or simply guessing a constant $0.5$.\cite{arieli_robust_2018}. 
% % A natural approach, and in fact a standard approach to the forecast aggregation problem in the literature, is the data-driven approach. 
% % The idea is simple.  

 
% % In practice, we hardly have access to an accurate prior. 
% % A standard approach in the forecast aggregation literature to overcoming this issue is the data-driven approach. 
% % The idea is simple: since many forecasting tasks are repeated (like the weather forecasting example above), we can collect samples of experts' predictions and the outcomes of the predicted event, and use those samples to find a good aggregation method accordingly.  For example, one can use a weighted average where each expert's weight is determined by historical data.

% % This data-driven approach has in fact been a standard approach in the forecast aggregation literature, with numerous empirical works studying how well different aggregation methods work in different real-world forecasting tasks.  See Section~\ref{sec:related_works} for discussions.



% % However, in reality, especially in the weather forecasting example above, the forecasting task is repeated every day, and the outcome of the event being predicted is observed (rain or not).  So, one can observe the historical forecasting performance of each expert and adjust the aggregation method accordingly.  For example, one can use a weighted average aggregation method where each expert's weight is determined by empirical data of its performance.  This data-driven approach has in fact been a standard approach in the forecast aggregation literature, with numerous empirical works studying how well different aggregation methods work in different real-world forecasting tasks.  See Section~\ref{sec:related_works} for discussions.

\subsection{Related Works}\label{sec:related_works}

\paragraph{Data-driven aggregation}
Data-driven approaches to forecast aggregation date back to perhaps the first paper on forecast aggregation (Bates and Granger, 1969, \cite{bates_combination_1969}) and have been standard in the literature (see, e.g., surveys \cite{clemen_combining_1989, timmermann_chapter_2006} and more recent works \cite{yang_combining_2004, satopaa_combining_2014, babichenko_learning_2021, wang_forecast_2021, frongillo_efficient_2021, neyman2022no}).  
Many of these works focus on specific weighted average aggregators like \emph{linear pooling} (weighted arithmetic mean) \cite{yang_combining_2004} and \emph{logarithmic pooling} (normalized weighted geometric mean) \cite{satopaa_combining_2014, neyman2022no}, and the goal is to estimate the optimal weights from data, which can usually be solved by standard statistical tools.  
However, those weighted average aggregators are not necessarily the optimal \emph{Bayesian} aggregator unless the underlying distribution $P$ of signals and event satisfies some strict assumptions (e.g., experts' forecasts are equal to the true probability of the event plus normally distributed noises \cite{winkler_combining_1981}).  For some distributions the performance of the Bayesian aggregator can be much better than the optimal weighted average. 
Our work aims to understand the sample complexity of Bayesian aggregation, namely how many samples are needed to approximate the Bayesian aggregator.  We think this is a fundamental question that should be addressed.


Our work is closely related to a recent work \cite{babichenko_learning_2021} on Bayesian aggregation via \emph{online learning}.  For the case of conditionally independent experts, \cite{babichenko_learning_2021} shows that the Bayesian aggregator can be approximated with $\eps = \tilde O(n\sqrt T)$ regret.  By an online-to-batch conversion (e.g., \cite{shalev-shwartz_online_2012}, Corollary 5.2), this implies a $T = \tilde O(\frac{n^2}{\eps^2})$ sample complexity upper bound in the batch learning setting.  We study the batch learning setting directly and obtain an improved bound of $\tilde O(\frac{n}{\eps^2})$.   
However, the loss function considered by \cite{babichenko_learning_2021} is different from ours: theirs is the logarithmic loss while ours is the squared loss.  Since the logarithmic loss is larger than the squared loss, their sample complexity bound should be greater than or equal to our bound.  We do not know whether there is a gap between the tight sample complexity bounds for the two loss functions. 


% \paragraph{Data-driven approaches to forecast aggregation and linear aggregation}
% Data-driven approaches to forecast aggregation already appeared in perhaps the first paper on forecast aggregation, \citet{bates_combination_1969}, and have been a standard practice in forecast aggregation (see, e.g., surveys by \citet{clemen_combining_1989} and \citet{timmermann_chapter_2006}). 
% Many of these works focus on weighted averaging, or more generally \emph{linear} aggregators, $f^{\bm \theta}(r_1, \ldots, r_n) = \sum_{i=1}^n \theta_i r_i + \theta_0$, studying how to use samples to estimate the best coefficient $\bm \theta$. 
% The use of linear aggregators is justified by the fact that the Bayesian optimal aggregator is indeed a linear function when the underlying distribution of experts' forecasts and the event satisfies some conditions, e.g., when experts' forecasts are the true probability of the event plus normally distributed noises (\citet{winkler_combining_1981}).
% While the restriction to linear aggregators and the assumption of normally distributed noise usually suffice for practical purposes, they do not necessarily capture the real underlying relationship between the event and the experts' forecasts.
% The Bayesian optimal aggregator is not linear in general, even for conditionally independent distributions (Section \ref{sec:conditionally_independent}).  
% Our work wants to understand how many samples are needed to approximately identify the Bayesian optimal aggregator.  We think this is a theoretically interesting and important question.
% Another reason why we do not restrict attentions to linear aggregators is that, once restricting to them, the aggregator learning problem reduces to a linear regression, and the sample complexity of aggregation becomes the sample complexity of linear regression, which is conceptually different from our purpose of understanding the sample complexity of aggregation \emph{itself}.
% While the sample complexity of linear aggregation has been studied by \citet{yang_combining_2004}, the sample complexity of Bayesian aggregation has not, as far as we know. 



\paragraph{Robust forecast aggregation}
Some recent works study the 
%There are also works on Bayesian aggregation that are not from a data-driven perspective
Bayesian aggregation problem \emph{not} from a data-driven perspective
\cite{frongillo_elicitation_2015, arieli_robust_2018, neyman_are_2021}.
In particular, \cite{arieli_robust_2018} and \cite{neyman_are_2021} study a ``robust forecast aggregation'' problem where the principal does not know and does not have samples from the prior distribution over experts' forecasts and the event.  They study the worst-case approximation ratio obtainable by a prior-free aggregator compared to the prior-aware Bayesian aggregator.  They give several negative results.  We are able to give positive results ($\eps$-approximation) because of two reasons: (1) we have sample access to the prior; (2) the Bayesian aggregator benchmark they choose is in fact stronger than ours; see Section~\ref{sec:model} for a detailed discussion. 

% problem  (e.g., \cite{arieli_robust_2018, babichenko_learning_2021, neyman_are_2021}) than the traditional forecasting literature (e.g., \cite{bates_combination_1969, morris_combining_1977, winkler_combination_1983, clemen_combining_1989, timmermann_chapter_2006}).
% The latter works usually assume a parametric family of distributions over the the ground truth and the experts' predictions.  Then, the learning task boils down to the estimation of parameters using historical data.

% Non-Bayesian approach: \cite{bates_combination_1969, newbold_experience_1974, winkler_combination_1983, granger_improved_1984}.
% Survey: \cite{clemen_combining_1989, timmermann_chapter_2006}. 

% \paragraph{No-regret learning}
% (e.g., \cite{cesa-bianchi_prediction_2006, frongillo_efficient_2021}) 

% Aggregating forecasts is different from aggregating signals \cite[p.198-199]{granger_improved_1984} \cite[p.168-169]{granger_invited_1989}, \cite[p.143]{timmermann_chapter_2006}. 

% Works about \emph{recalibration} (e.g., \cite{turner_forecast_2014, budescu_identifying_2015}) also study how to choose aggregators based on experts' historical performance.  But those works are mainly empirical: they evaluate the performance of specific aggregator-choosing schemes based on real-world data, without sample complexity analysis.  

\paragraph{Sample complexity of mechanism design}  Our work may remind the reader of a long line of research on the sample complexity of mechanism design, in particular revenue maximization (e.g., \cite{cole_sample_2014, dhangwatnotai_revenue_2015, morgenstern_pseudo-dimension_2015, devanur_sample_2016, balcan_sample_2016, cai_learning_2017, guo_settling_2019, brustle_multi-item_2020, gonczarowski_sample_2021, guo_generalizing_2021}).  A key observation from these works is that, the number of samples needed to learn an $\eps$-optimal auction for $n\ge 1$ independent bidders is increasing in $n$, because when there are more bidders, although we can obtain higher revenue, the optimal auction benchmark also gets improved.  We see a similar phenomenon in the forecast aggregation problem where the sample complexity increases with the number of experts in the general case, but we do not know whether this phenomenon persists when experts are conditionally independent. 



==> intro_v4.tex <==
\section{Introduction} 
Suppose you want to know whether it will rain tomorrow.  You search ``weather'' on Google, and it says that the probability of raining tomorrow is 40\%.  But the weather forecasting app on your phone shows 85\%.  And one of your friends, who is an expert in meteorology, predicts 65\%.  How do you aggregate these predictions into a single one?  
This problem is called \emph{forecast aggregation} or \emph{forecast combination} (e.g., \cite{bates_combination_1969, clemen_combining_1989, timmermann_chapter_2006}).
It has innumerable applications in fields ranging from economics, statistics, operations research, to machine learning, decision theory, and of course, climate science. 

% A known phenomenon in many empirical works on forecast aggregation is the ``forecast combination puzzle'' \cite[p.428]{stock_combination_2004}: a simple aggregation methods like the unweighted averaging of all experts' forecasts often outperform more sophisticated, data-driven, aggregation methods. 

A straightforward solution to the forecast aggregation problem is simply taking the (unweighted) average of all experts' forecasts.
This method does not take into account, for example, the fact that different experts may have different expertise. 
One can naturally think of more sophisticated aggregators, like weighted averages.  In particular, a standard approach to forecast aggregation in the literature is the \emph{data-driven} approach (see Related Works for details): since many forecasting tasks are repetitive, one can first collect experts' forecasts and the realizations of the predicted events in the past, then use those data to learn an aggregator for future forecasting tasks.  For example, one can try weighted averages where the weights of experts are determined by their historical prediction accuracy, or even train neural network aggregators.
How do these data-driven methods compare to the simple unweighted average? 

Interestingly, though, as observed consistently by forecast aggregation works from 1960s to 2020s (e.g., \cite{bates_combination_1969, newbold_experience_1974, makridakis_averages_1983, winkler_combination_1983, gupta_combination_1987, clemen_combining_1989, stock_combination_2004, timmermann_chapter_2006, genre_combining_2013, makridakis_m4_2020}), many sophisticated data-driven aggregation methods actually perform \emph{worse} than the simple average in practice. 
For instance, while the weighted averaging methods with weights determined by experts' individual accuracy are sometimes better than the simple average, those taking into account the correlations between experts are usually worse \cite{winkler_combination_1983}. 
The dominance of simple average over sophisticated data-driven methods appeared so often in practice that it has been known as ``the forecast combination puzzle'' in the literature \cite[p.428]{stock_combination_2004}.
Explanations to this puzzle have been given, and a widely accepted one is, unsurprisingly, \emph{overfitting} \cite{smith_simple_2009, genre_combining_2013, claeskens_forecast_2016}: 
optimizing a sophisticated data-driven method usually requires a large amount of data, which are hard to obtain in practice. 

When we look at the sample sizes in works that support the simple average, however, they are pretty small in today's ``big-data'' standard (24 in \cite{granger_improved_1984}, 69 in \cite{satopaa_combining_2014}, 87 in \cite{baron_two_2014}, 100 in \cite{gupta_combination_1987}).  
Admittedly, data are difficult to obtain when human experts are involved.  But in many modern algorithm-driven forecasting tasks we do have access to large amounts of data.  Weather forecast is one example, where we have forecasts made by algorithms on different days at different locations.  Online forecasting competition platforms like Kaggle also generate abundant data.\footnote{\url{https://www.kaggle.com/c/m5-forecasting-accuracy}}  In those scenarios, one should expect some sophisticated data-driven methods to outperform the simple average by a lot.  Taking a step further, one might wonder:  What is the \emph{best} aggregation we can hopefully achieve if we are given infinite data?  How many data/samples do we need to approximately achieve that? 
These questions motivate our work.

% 
% Even when we do not have a large amount of samples, our understanding of the forecast combination puzzle is still largely empirical.  Few works have theoretically answered the following question: how many samples do we need to outperform the simple averaging? 
% 
% Using terminologies from statistical learning theory \cite{vapnik_nature_2000}, we call this problem ``the sample complexity of forecast aggregation''.

\paragraph{Our contributions}
We initiate the study of \emph{sample complexity of forecast aggregation}, namely:  
\begin{center}
    \emph{How many samples do we need to achieve the optimal aggregation approximately?}
\end{center} 

Our first result shows that the sample complexity of forecast aggregation can be extremely large in the worst case.  This partly explains why sophisticated data-driven methods hardly outperform the simple averaging.  Specifically, we consider a standard Bayesian forecast model (first developed by \cite{morris_decision_1974, winkler_combining_1981}, surveyed in \cite{geweke_chapter_2006}) as follows: there are $n$ experts, one principal; each expert $i$ observes a private signal $s_i \in \S_i$ about an unknown binary event (state of the world) $\omega\in\{0, 1\}$; experts' signals and the event jointly follow an underlying distribution $P$; each expert reports their posterior belief $r_i = P(\omega = 1 \,|\, s_i)$ about $\omega$ to the principal, who then aggregates all the reports $r_1, \ldots, r_n$ into a single prediction for $\omega$.
We assume that the principal does not know $P$ but has i.i.d.~samples of experts' reports (not signals) and event realizations from $P$, based on which it wants to find an aggregator $\hat f: [0, 1]^n \to [0, 1]$ that is ``$\eps$-close'' to the ``optimal'' aggregator $f^*$ (we define ``optimal'' in Section~\ref{sec:model}), which is the Bayesian aggregator $f^*(r_1, \ldots, r_n) = P(\omega = 1 \,|\, r_1, \ldots, r_n)$, where ``$\eps$-closeness'' is measured in the mean squared difference: $\E_P\big[|\hat f(r_1, \ldots, r_n) - f^*(r_1, \ldots, r_n)|^2\big]\le \eps$. 
Assuming a finite signal space of size $|\S_i| = m$ for each expert, we show that: 
\begin{itemize}
    \item To find an aggregator $\hat f$ that is $\eps$-close to the optimal aggregator $f^*$ with high probability for any distribution $P$, at most $\tilde O(\frac{m^{n}}{\eps^2})$ samples are sufficient, and at least $\tilde \Omega(\frac{m^{n-2}}{\eps})$ samples are necessary.\footnote{The $\tilde O(\cdot)$ and $\tilde \Omega(\cdot)$ notations omit logarithmic factors.} (Theorem~\ref{thm:general_distribution_both}.)
\end{itemize}
% This exponential number of samples is never practical, thus supporting the forecast combination puzzle that empirically learned aggregators could be outperformed by a simple averaging in practice.  We also provide an $O(\frac{m^n}{\eps^2})$ sample complexity upper bound (Theorem~\ref{thm:general_distribution_upper_bound}).  Both the lower bound and the upper bound hold for general distribution $P$. 

The exponential sample complexity lower bound $\tilde \Omega(\frac{m^{n-2}}{\eps})$ means that the optimal aggregator $f^*$ is rather difficult to learn, and significantly more difficult when the number of experts increases.  As we show in the proof (which is a reduction from the \emph{distribution learning} problem), this difficulty stems from the fact that we need to estimate the correlation between experts, which requires a large number of samples.
This motivates us to study the special case where (the signals of) experts are conditionally independent, namely, $s_i$'s are independent conditioning on $\omega$. 
The sample complexity is significantly reduced in this case:
\begin{itemize}
    \item If experts are conditionally independent, then an $\eps$-optimal aggregator $\hat f$ can be found with high probability using only $\tilde O(\frac{n}{\eps^2})$ samples.  $\tilde \Omega(\frac{1}{\eps})$ samples are necessary. (Theorem~\ref{thm:conditionally_independent_general}.)
\end{itemize}

The sample complexity upper bound $\tilde O(\frac{n}{\eps^2})$ in the conditionally independent case is only linear in $n$ and independent of the signal space size $m$.  
We then further investigate two special conditionally independent cases where the experts are either ``very informative'' or ``very non-informative''.  Under both cases the sample complexity can be $\tilde O(\frac{1}{\eps})$ or even smaller (Theorem~\ref{thm:strongly-informative-upper-bound} and \ref{thm:weakly-informative-upper-bound:new}). 


% The significant gap between the sample complexity for general distributions and conditionally independent distributions suggests another form of ``forecast combination puzzle'': aggregation methods that ignore the correlation between experts could perform better than those that take the correlation into account, given a practical sample size.  This phenomenon has actually been observed by empirical works on forecast aggregation \cite{makridakis_averages_1983, gupta_combination_1987, stock_combination_2004}.  Our results hence provide a quantitative theoretical explanation to this phenomenon. 

We review related works in Section~\ref{sec:related_works}.  Section~\ref{sec:model} introduces model and preliminary. 
Section~\ref{sec:general_distribution} studies the sample complexity for general distributions.  Section~\ref{sec:conditionally_independent} considers the conditionally independent case.  Section~\ref{sec:conclusion} concludes and discusses future directions. 

% \paragraph{Structure of the paper}
% We review related works next.  Models and preliminaries are in Section~\ref{sec:model}.  

% \subsection{Overview of Our Results}
% \paragraph{Model} 
% To formalize the sample complexity question above, we consider the following forecast aggregation model, which is a Bayesian framework proposed by Morris (1974) \cite{morris_decision_1974} and more recently studied by \cite{arieli_robust_2018, babichenko_learning_2021, neyman_are_2021}: A principal wants to predict the unknown state of the world $\omega \in \{0, 1\}$.  There are $n$ experts, each observing a private signal $s_i \in \S_i$ that correlates with the state of the world according to some underlying distribution $P$.  Experts know (their marginals of) the distribution $P$ and report their posterior beliefs about $\omega$ to the principal: $r_i = P(\omega = 1 \mid s_i)$.  Given the reports $\bm r = (r_1, \ldots, r_n)$, the principal aggregates them into a single prediction $f(r_1, \ldots, r_n) \in [0, 1]$.  Crucially, we assume that the distribution $P$ is unknown to the principal and can be arbitrarily chosen.  If the principal knows $P$, then it can aggregate ``optimally'' (we formally define ``optimality'' in Section~\ref{sec:model}) using the Bayes' rule: compute the posterior probability of $\omega = 1$ given all the information it receives, $f^*(r_1, \ldots, r_n) = P(\omega = 1 \mid r_1, \ldots, r_n)$.

% The principal has access to $T$ i.i.d.~samples of reports and the realization of the state of the world according to $P$: 
% \begin{equation*}
%     (\bm r^{(1)}, \omega^{(1)}), (\bm r^{(2)}, \omega^{(2)}), ~ \ldots, ~ (\bm r^{(T)}, \omega^{(T)}),  \quad \quad \bm r^{(t)} = (r_1^{(t)}, \ldots, r_n^{(t)}),  
% \end{equation*}
% using which it finds an aggregator $\hat f: [0, 1]^n \to [0, 1]$. 
% An aggregator is $\eps$-optimal if its mean squared difference with $f^*$ is less than $\eps$, where the mean is with respect to $P$: $\E_P\big[|f(\bm r) - f^*(\bm r)|^2\big]\le \eps$. 
% Now, the sample complexity question can be rephrased as follows: 
% \begin{center}
% \emph{How many samples are necessary and sufficient for finding an $\eps$-optimal aggregator \\
% (with high probability over the random draw of samples)?} 
% \end{center}

% \paragraph{Results}
% Unlike many forecast aggregation works that restrict attentions to linear aggregators $\hat f(\bm r) = \sum_{i=1}^n a_i r_i$, we do not put such restrictions on $\hat f$, because we want to approximate the optimal aggregator $f^*$ which need not be linear.  However, such approximation cannot be done with a finite number of samples if $P$ can be an arbitrary continuous distribution.  Hence, our work makes two types of assumptions on $P$: (1) \emph{discrete signal space}: each $\S_i$ is a finite set of size $m < \infty$; (2) \emph{conditionally independent signals}: $s_1, \ldots, s_n$ are independently distributed conditioning on $\omega$.  We prove that, under these assumptions, an $\eps$-optimal aggregator can be found with a finite number of samples.  Specifically, the number of samples is upper bounded by: 
% \begin{itemize}
%     \item Discrete signal space: $O\big(\frac{m^n}{\eps^2}\big)$ (Theorem~\ref{thm:general_distribution_upper_bound}). 
%     \item Conditionally independent signals: $O\big(\frac{(n-1)^2}{\rho \eps}\big)$, where $\rho = \frac{P(\omega = 1)}{P(\omega = 0)}$ is a constant (Theorem~\ref{thm:conditionally_independent_upper_bound}). 
% \end{itemize}

% The above two results answer the ``sufficient'' part in the question we raised above.  The more interesting, and more challenging, part is how many samples are ``necessary''?  We show that, in order to obtain $\eps$-optimal aggregators with high probability, one needs at least the following numbers of samples: 
% \begin{itemize}
%     \item Discrete signal space: $\Omega\big(\frac{m^{n-2}}{\eps}\big)$ (Theorem~\ref{thm:general_distribution_lower_bound}). 
%     \item Conditionally independent signals: $\Omega\big(\frac{1}{\eps}\big)$ (Theorem~\ref{thm:conditionally_independent_lower_bound}). 
% \end{itemize}

% \paragraph{Discussion}
% The exponential sample complexity of learning $\eps$-optimal aggregators for distributions over discrete signal space basically means that learning the optimal aggregator is rather difficult.  As we show in the proof, this difficulty stems from the fact that we need to estimate the correlations between experts.  To estimate such correlations with ``$\eps$-accuracy'', we need $\Omega\big(\frac{m^{n-2}}{\eps}\big)$ samples.
% In practice, this number of samples can hardly be obtained.

% However, once we assume that experts are conditionally independent, the sample complexity significantly reduces.  This could suggest another form of ``forecast combination puzzle'': aggregation methods that ignore the correlations between experts could perform better than those take into account correlations, given a practical number of samples.  This phenomenon has been observed by empirical works \cite{makridakis_averages_1983, gupta_combination_1987, stock_combination_2004}.  Our results provide a rigorous theoretical explanation to this phenomenon. 


% % ===================================================

% % The role of \emph{prior} is important in the forecast aggregation problem. 
% % If we do not have any prior knowledge about the weather or the experts' predicting abilities, then the best we could do is basically some trivial aggregation methods, like taking the average of the experts' predictions, or simply guessing a constant $0.5$.\cite{arieli_robust_2018}. 
% % A natural approach, and in fact a standard approach to the forecast aggregation problem in the literature, is the data-driven approach. 
% % The idea is simple.  

 
% % In practice, we hardly have access to an accurate prior. 
% % A standard approach in the forecast aggregation literature to overcoming this issue is the data-driven approach. 
% % The idea is simple: since many forecasting tasks are repeated (like the weather forecasting example above), we can collect samples of experts' predictions and the outcomes of the predicted event, and use those samples to find a good aggregation method accordingly.  For example, one can use a weighted average where each expert's weight is determined by historical data.

% % This data-driven approach has in fact been a standard approach in the forecast aggregation literature, with numerous empirical works studying how well different aggregation methods work in different real-world forecasting tasks.  See Section~\ref{sec:related_works} for discussions.



% % However, in reality, especially in the weather forecasting example above, the forecasting task is repeated every day, and the outcome of the event being predicted is observed (rain or not).  So, one can observe the historical forecasting performance of each expert and adjust the aggregation method accordingly.  For example, one can use a weighted average aggregation method where each expert's weight is determined by empirical data of its performance.  This data-driven approach has in fact been a standard approach in the forecast aggregation literature, with numerous empirical works studying how well different aggregation methods work in different real-world forecasting tasks.  See Section~\ref{sec:related_works} for discussions.

\subsection{Related Works}\label{sec:related_works}

\paragraph{Data-driven aggregation}
Data-driven approaches to forecast aggregation date back to perhaps the first paper on forecast aggregation (Bates and Granger, 1969, \cite{bates_combination_1969}) and have been standard in the literature (see, e.g., surveys \cite{clemen_combining_1989, timmermann_chapter_2006} and more recent works \cite{yang_combining_2004, satopaa_combining_2014, babichenko_learning_2021, wang_forecast_2021, frongillo_efficient_2021, neyman2022no}).  
Many of these works focus on specific weighted average aggregators like \emph{linear pooling} (weighted arithmetic mean) \cite{yang_combining_2004} and \emph{logarithmic pooling} (normalized weighted geometric mean) \cite{satopaa_combining_2014, neyman2022no}, and the goal is to estimate the optimal weights from data, which can usually be solved by standard statistical tools.  
However, those weighted average aggregators are not necessarily the optimal \emph{Bayesian} aggregator unless the underlying distribution $P$ of signals and event satisfies some strict assumptions (e.g., experts' forecasts are equal to the true probability of the event plus normally distributed noises \cite{winkler_combining_1981}).  For some distributions the performance of the Bayesian aggregator can be much better than the optimal weighted average. 
Our work aims to understand the sample complexity of Bayesian aggregation, namely how many samples are needed to approximate the Bayesian aggregator.  We think this is a fundamental question that should be addressed.


Our work is closely related to a recent work \cite{babichenko_learning_2021} on Bayesian aggregation via \emph{online learning}.  For the case of conditionally independent experts, \cite{babichenko_learning_2021} shows that the Bayesian aggregator can be approximated with $\eps = \tilde O(n\sqrt T)$ regret.  By an online-to-batch conversion (e.g., \cite{shalev-shwartz_online_2012}, Corollary 5.2), this implies a $T = \tilde O(\frac{n^2}{\eps^2})$ sample complexity upper bound in the batch learning setting.  We study the batch learning setting directly and obtain an improved bound of $\tilde O(\frac{n}{\eps^2})$.   
However, the loss function considered by \cite{babichenko_learning_2021} is different from ours: theirs is the logarithmic loss while ours is the squared loss.  Since the logarithmic loss is larger than the squared loss, their sample complexity bound should be greater than or equal to our bound.  We do not know whether there is a gap between the tight sample complexity bounds for the two loss functions. 


% \paragraph{Data-driven approaches to forecast aggregation and linear aggregation}
% Data-driven approaches to forecast aggregation already appeared in perhaps the first paper on forecast aggregation, \citet{bates_combination_1969}, and have been a standard practice in forecast aggregation (see, e.g., surveys by \citet{clemen_combining_1989} and \citet{timmermann_chapter_2006}). 
% Many of these works focus on weighted averaging, or more generally \emph{linear} aggregators, $f^{\bm \theta}(r_1, \ldots, r_n) = \sum_{i=1}^n \theta_i r_i + \theta_0$, studying how to use samples to estimate the best coefficient $\bm \theta$. 
% The use of linear aggregators is justified by the fact that the Bayesian optimal aggregator is indeed a linear function when the underlying distribution of experts' forecasts and the event satisfies some conditions, e.g., when experts' forecasts are the true probability of the event plus normally distributed noises (\citet{winkler_combining_1981}).
% While the restriction to linear aggregators and the assumption of normally distributed noise usually suffice for practical purposes, they do not necessarily capture the real underlying relationship between the event and the experts' forecasts.
% The Bayesian optimal aggregator is not linear in general, even for conditionally independent distributions (Section \ref{sec:conditionally_independent}).  
% Our work wants to understand how many samples are needed to approximately identify the Bayesian optimal aggregator.  We think this is a theoretically interesting and important question.
% Another reason why we do not restrict attentions to linear aggregators is that, once restricting to them, the aggregator learning problem reduces to a linear regression, and the sample complexity of aggregation becomes the sample complexity of linear regression, which is conceptually different from our purpose of understanding the sample complexity of aggregation \emph{itself}.
% While the sample complexity of linear aggregation has been studied by \citet{yang_combining_2004}, the sample complexity of Bayesian aggregation has not, as far as we know. 



\paragraph{Robust forecast aggregation}
Some recent works study the 
%There are also works on Bayesian aggregation that are not from a data-driven perspective
Bayesian aggregation problem \emph{not} from a data-driven perspective
\cite{frongillo_elicitation_2015, arieli_robust_2018, neyman_are_2021}.
In particular, \cite{arieli_robust_2018} and \cite{neyman_are_2021} study a ``robust forecast aggregation'' problem where the principal does not know and does not have samples from the prior distribution over experts' forecasts and the event.  They study the worst-case approximation ratio obtainable by a prior-free aggregator compared to the prior-aware Bayesian aggregator.  They give several negative results.  We are able to give positive results ($\eps$-approximation) because of two reasons: (1) we have sample access to the prior; (2) the Bayesian aggregator benchmark they choose is in fact stronger than ours; see Section~\ref{sec:model} for a detailed discussion. 

% problem  (e.g., \cite{arieli_robust_2018, babichenko_learning_2021, neyman_are_2021}) than the traditional forecasting literature (e.g., \cite{bates_combination_1969, morris_combining_1977, winkler_combination_1983, clemen_combining_1989, timmermann_chapter_2006}).
% The latter works usually assume a parametric family of distributions over the the ground truth and the experts' predictions.  Then, the learning task boils down to the estimation of parameters using historical data.

% Non-Bayesian approach: \cite{bates_combination_1969, newbold_experience_1974, winkler_combination_1983, granger_improved_1984}.
% Survey: \cite{clemen_combining_1989, timmermann_chapter_2006}. 

% \paragraph{No-regret learning}
% (e.g., \cite{cesa-bianchi_prediction_2006, frongillo_efficient_2021}) 

% Aggregating forecasts is different from aggregating signals \cite[p.198-199]{granger_improved_1984} \cite[p.168-169]{granger_invited_1989}, \cite[p.143]{timmermann_chapter_2006}. 

% Works about \emph{recalibration} (e.g., \cite{turner_forecast_2014, budescu_identifying_2015}) also study how to choose aggregators based on experts' historical performance.  But those works are mainly empirical: they evaluate the performance of specific aggregator-choosing schemes based on real-world data, without sample complexity analysis.  

\paragraph{Sample complexity of mechanism design}  Our work may remind the reader of a long line of research on the sample complexity of mechanism design, in particular revenue maximization (e.g., \cite{cole_sample_2014, dhangwatnotai_revenue_2015, morgenstern_pseudo-dimension_2015, devanur_sample_2016, balcan_sample_2016, cai_learning_2017, guo_settling_2019, brustle_multi-item_2020, gonczarowski_sample_2021, guo_generalizing_2021}).  A key observation from these works is that, the number of samples needed to learn an $\eps$-optimal auction for $n\ge 1$ independent bidders is increasing in $n$, because when there are more bidders, although we can obtain higher revenue, the optimal auction benchmark also gets improved.  We see a similar phenomenon in the forecast aggregation problem where the sample complexity increases with the number of experts in the general case, but we do not know whether this phenomenon persists when experts are conditionally independent. 



==> intro_v5.tex <==
\section{Introduction} 
Suppose you want to know whether it will rain tomorrow.  A Google search on ``weather'' returns 40\% probability of raining for tomorrow. The weather forecasting app on your phone shows 85\%.  And one of your friends, who is an expert in meteorology, predicts 65\%.  How do you aggregate these different predictions into a single, accurate prediction?  
This problem is called \emph{forecast aggregation} or \emph{forecast combination} \cite{bates_combination_1969, clemen_combining_1989, timmermann_chapter_2006}.
It has innumerable applications in fields ranging from economics, statistics, operations research, to machine learning, decision theory, and of course, climate science. 

\yc{Tao, could you please fill in the missing citations and also check whether I put the references at the appropriate places?}
% A known phenomenon in many empirical works on forecast aggregation is the ``forecast combination puzzle'' \cite[p.428]{stock_combination_2004}: a simple aggregation methods like the unweighted averaging of all experts' forecasts often outperform more sophisticated, data-driven, aggregation methods. 

A straightforward solution to forecast aggregation is to simply take the (unweighted) average of all experts' forecasts. Simple as it is, unweighted average performs surprisingly well in practice, as observed by many forecast aggregation works from 1960s to 2020s (e.g., \cite{bates_combination_1969, newbold_experience_1974, makridakis_averages_1983, gupta_combination_1987, clemen_combining_1989, timmermann_chapter_2006, makridakis_m4_2020}). 
Naturally, when past data of expert forecasts and event outcomes (e.g., historical weather forecasts and outcomes) are available, one may hope to leverage on such data to learn more accurate aggregators. While adjusting weights of experts in averaging according to their individual historical accuracy has led to improved accuracy for the aggregated prediction~\cite{winkler_combination_1983}, interestingly,
% more sophisticated data-driven aggregation methods, including accounting for correlation of experts when setting their weights \cite{winkler_combination_1983} and training neural network aggregators []
\yc{I wonder whether a more ML example is better} 
\tl{maybe we should not mention neural networks here.  I didn't find evidence showing that neural networks aggregators are worse than simple average. }
more sophisticated data-driven methods like adjusting the weights using ordinary least squared regression \cite{genre_combining_2013} and covariance estimation \cite{makridakis_averages_1983, winkler_combination_1983} were often outperformed by the unweighted average.
%\cite{gupta_combination_1987, stock_combination_2004, genre_combining_2013}.
The dominance of simple aggregators over more sophisticated data-driven methods is observed so often in empirical applications that it is termed ``the forecast combination puzzle'' \cite[p.428]{stock_combination_2004}.

%This ‘forecast combination puzzle’—the repeated finding that simple combination forecasts outperform sophisticated adaptive combination methods in empirical appli- cations

There are many potential explanations for the forecast combination puzzle~\cite{smith_simple_2009, genre_combining_2013, claeskens_forecast_2016}. In some scenarios, the past events are different from the future events in fundamental ways (e.g., geopolitical forecasting) and hence past data may not be informative in predicting the future. Another widely accepted conjecture is that the amount of past data is not large enough for a data-intensive method to % learn an accurate aggregator.
perform well.
% Indeed, the sample sizes in works that support the simple average are small under today's ``big-data'' standard (24 in \cite{granger_improved_1984}, 69 in \cite{satopaa_combining_2014},87 in \cite{baron_two_2014}, 100 in \cite{gupta_combination_1987}).
Indeed, the sample sizes in many empirical forecast aggregation works are small under today's ``big-data'' standard (24 in \cite{granger_improved_1984}, 69 in \cite{satopaa_combining_2014}, 87 in \cite{baron_two_2014}, 100 in \cite{gupta_combination_1987}).
However, there are aggregation settings where it is reasonable to think that future events are similar to past events and we do have abundant data --- 
%for instance, weather forecasting and some forecasting competitions on Kaggle\footnote{\url{https://www.kaggle.com/c/m5-forecasting-accuracy}}. Such settings are well-suited for data-driven methods.
for instance, the forecasting of weather, stock prices \cite{donaldson_forecast_1996}, and some forecasting competitions on Kaggle\footnote{\url{https://www.kaggle.com/c/m5-forecasting-accuracy}}. Such settings are well-suited for data-driven methods.
In fact, when given enough data, neural network based nonlinear aggregators can perform better than traditional linear aggregators \cite{donaldson_forecast_1996, ming_shi_improving_1999, wang_optimal_2018}.
\tl{Added citations for neural network aggregators}
It's hence tempting to ask \emph{how many} data are needed for data-driven aggregators to achieve high accuracy in these settings. 

\yc{In the current version, I didn't talk about overfitting. Is it ok to omit it? Maybe we can find a different place to cite \cite{smith_simple_2009, genre_combining_2013, claeskens_forecast_2016}.}
\tl{I think it's OK to omit it.  And just put them after the first sentence ``there are many potential explanations xxx''? }\yc{OK. Added the citations.}

In this paper, we initiate the study of \emph{sample complexity of forecast aggregation}, building upon a standard Bayesian forecasting model \cite{morris_decision_1974, winkler_combining_1981, geweke_chapter_2006}.
\tl{Add brief description of the model}
In this model, the optimal aggregator (which is Bayesian) depends on an underlying unknown joint distribution of the experts' reports and the event outcome, from which we obtain samples.  
\tl{I'm a bit confused by the two ``models'' here.  Maybe no need to say ``in a statistical learning model''? } \yc{I removed statistical learning model. The batch learning perspective, that is, we have samples and want to learn an aggregator, is what I mean by a statistical learning model. I don't think the standard Bayesian forecasting model has the learning aspect.}
We ask:
\begin{center}
    \emph{How many samples do we need to approximately learn the optimal Bayesian aggregator?}
\end{center} 
We show that the sample complexity of forecast aggregation can be extremely large in the worst case. But it is significantly lower for some special families of distributions. \tl{Should we say information structure or distributions?}\yc{Changed it to distributions for consistency.}
Our results provide partial explanation for the observed forecast combination puzzle. 

\paragraph{Main results} 
In our model, there are $n$ experts and one principal. Each expert $i$ observes a private signal $s_i \in \S_i$ about an unknown binary event (state of the world) $\omega\in\{0, 1\}$. Experts' signals and the event jointly follow an underlying distribution $P$. Each expert reports their posterior belief $r_i = P(\omega = 1 \,|\, s_i)$ about $\omega$ to the principal, who then aggregates all the reports $r_1, \ldots, r_n$ into a single prediction for $\omega$.
The principal does not know $P$ but has i.i.d.~``samples'' from the distribution, where each sample is a tuple
of experts' reports (not signals) and the realization of the event. Using these samples, the principal aims to find an aggregator $\hat f: [0, 1]^n \to [0, 1]$ that is ``$\eps$-close'' to the optimal Bayesian aggregator $f^*(r_1, \ldots, r_n) = P(\omega = 1 \,|\, r_1, \ldots, r_n)$, where ``$\eps$-closeness'' is measured in the mean squared difference: $\E_P\big[|\hat f(r_1, \ldots, r_n) - f^*(r_1, \ldots, r_n)|^2\big]\le \eps$. 

Assuming a finite signal space of size $|\S_i| = m$ for each expert, we show that: 
\begin{itemize}
    \item To find an aggregator $\hat f$ that is $\eps$-close to the optimal aggregator $f^*$ with high probability for any distribution $P$, at most $\tilde O(\frac{m^{n}}{\eps^2})$ samples are sufficient, and at least $\tilde \Omega(\frac{m^{n-2}}{\eps})$ samples are necessary.\footnote{The $\tilde O(\cdot)$ and $\tilde \Omega(\cdot)$ notations omit logarithmic factors.} (Theorem~\ref{thm:general_distribution_both}.)
\end{itemize}
% This exponential number of samples is never practical, thus supporting the forecast combination puzzle that empirically learned aggregators could be outperformed by a simple averaging in practice.  We also provide an $O(\frac{m^n}{\eps^2})$ sample complexity upper bound (Theorem~\ref{thm:general_distribution_upper_bound}).  Both the lower bound and the upper bound hold for general distribution $P$. 

The exponential sample complexity lower bound $\tilde \Omega(\frac{m^{n-2}}{\eps})$ means that the optimal aggregator $f^*$ is rather difficult to learn, and significantly more difficult when the number of experts increases.  As we show in the proof (which is a reduction from the \emph{distribution learning} problem), this difficulty stems from the fact that we need to estimate the correlation between experts, which requires a large number of samples.
This motivates us to study the special case where (the signals of) experts are conditionally independent, namely, $s_i$'s are independent conditioned on $\omega$. 
The sample complexity is significantly reduced in this case:
\begin{itemize}
    \item If experts are conditionally independent, then an $\eps$-optimal aggregator $\hat f$ can be found with high probability using only $\tilde O(\frac{1}{\eps^2})$ samples.  $\tilde \Omega(\frac{1}{\eps})$ samples are necessary. (Theorem~\ref{thm:conditionally_independent_general}.)
\end{itemize}

The sample complexity upper bound $\tilde O(\frac{1}{\eps^2})$ in the conditional independence case does not depend on the number of agents $n$ and the signal space size $m$.  
We then further investigate two special conditional independence cases where the experts are either ``very informative'' or ``very non-informative''.  In both cases the sample complexity can be $\tilde O(\frac{1}{\eps})$ or even smaller (Theorem~\ref{thm:strongly-informative-upper-bound} and \ref{thm:weakly-informative-upper-bound:new}). 

In the remainder of the paper, we first discuss related works in Section~\ref{sec:related_works}.  Section~\ref{sec:model} introduces our model and preliminaries. 
Section~\ref{sec:general_distribution} studies the sample complexity for general distributions.  Section~\ref{sec:conditionally_independent} focuses on the conditional independence case.  We conclude and discuss future directions in Section~\ref{sec:conclusion}. 

% \paragraph{Structure of the paper}
% We review related works next.  Models and preliminaries are in Section~\ref{sec:model}.  

% \subsection{Overview of Our Results}
% \paragraph{Model} 
% To formalize the sample complexity question above, we consider the following forecast aggregation model, which is a Bayesian framework proposed by Morris (1974) \cite{morris_decision_1974} and more recently studied by \cite{arieli_robust_2018, babichenko_learning_2021, neyman_are_2021}: A principal wants to predict the unknown state of the world $\omega \in \{0, 1\}$.  There are $n$ experts, each observing a private signal $s_i \in \S_i$ that correlates with the state of the world according to some underlying distribution $P$.  Experts know (their marginals of) the distribution $P$ and report their posterior beliefs about $\omega$ to the principal: $r_i = P(\omega = 1 \mid s_i)$.  Given the reports $\bm r = (r_1, \ldots, r_n)$, the principal aggregates them into a single prediction $f(r_1, \ldots, r_n) \in [0, 1]$.  Crucially, we assume that the distribution $P$ is unknown to the principal and can be arbitrarily chosen.  If the principal knows $P$, then it can aggregate ``optimally'' (we formally define ``optimality'' in Section~\ref{sec:model}) using the Bayes' rule: compute the posterior probability of $\omega = 1$ given all the information it receives, $f^*(r_1, \ldots, r_n) = P(\omega = 1 \mid r_1, \ldots, r_n)$.

% The principal has access to $T$ i.i.d.~samples of reports and the realization of the state of the world according to $P$: 
% \begin{equation*}
%     (\bm r^{(1)}, \omega^{(1)}), (\bm r^{(2)}, \omega^{(2)}), ~ \ldots, ~ (\bm r^{(T)}, \omega^{(T)}),  \quad \quad \bm r^{(t)} = (r_1^{(t)}, \ldots, r_n^{(t)}),  
% \end{equation*}
% using which it finds an aggregator $\hat f: [0, 1]^n \to [0, 1]$. 
% An aggregator is $\eps$-optimal if its mean squared difference with $f^*$ is less than $\eps$, where the mean is with respect to $P$: $\E_P\big[|f(\bm r) - f^*(\bm r)|^2\big]\le \eps$. 
% Now, the sample complexity question can be rephrased as follows: 
% \begin{center}
% \emph{How many samples are necessary and sufficient for finding an $\eps$-optimal aggregator \\
% (with high probability over the random draw of samples)?} 
% \end{center}

% \paragraph{Results}
% Unlike many forecast aggregation works that restrict attentions to linear aggregators $\hat f(\bm r) = \sum_{i=1}^n a_i r_i$, we do not put such restrictions on $\hat f$, because we want to approximate the optimal aggregator $f^*$ which need not be linear.  However, such approximation cannot be done with a finite number of samples if $P$ can be an arbitrary continuous distribution.  Hence, our work makes two types of assumptions on $P$: (1) \emph{discrete signal space}: each $\S_i$ is a finite set of size $m < \infty$; (2) \emph{conditionally independent signals}: $s_1, \ldots, s_n$ are independently distributed conditioning on $\omega$.  We prove that, under these assumptions, an $\eps$-optimal aggregator can be found with a finite number of samples.  Specifically, the number of samples is upper bounded by: 
% \begin{itemize}
%     \item Discrete signal space: $O\big(\frac{m^n}{\eps^2}\big)$ (Theorem~\ref{thm:general_distribution_upper_bound}). 
%     \item Conditionally independent signals: $O\big(\frac{(n-1)^2}{\rho \eps}\big)$, where $\rho = \frac{P(\omega = 1)}{P(\omega = 0)}$ is a constant (Theorem~\ref{thm:conditionally_independent_upper_bound}). 
% \end{itemize}

% The above two results answer the ``sufficient'' part in the question we raised above.  The more interesting, and more challenging, part is how many samples are ``necessary''?  We show that, in order to obtain $\eps$-optimal aggregators with high probability, one needs at least the following numbers of samples: 
% \begin{itemize}
%     \item Discrete signal space: $\Omega\big(\frac{m^{n-2}}{\eps}\big)$ (Theorem~\ref{thm:general_distribution_lower_bound}). 
%     \item Conditionally independent signals: $\Omega\big(\frac{1}{\eps}\big)$ (Theorem~\ref{thm:conditionally_independent_lower_bound}). 
% \end{itemize}

% \paragraph{Discussion}
% The exponential sample complexity of learning $\eps$-optimal aggregators for distributions over discrete signal space basically means that learning the optimal aggregator is rather difficult.  As we show in the proof, this difficulty stems from the fact that we need to estimate the correlations between experts.  To estimate such correlations with ``$\eps$-accuracy'', we need $\Omega\big(\frac{m^{n-2}}{\eps}\big)$ samples.
% In practice, this number of samples can hardly be obtained.

% However, once we assume that experts are conditionally independent, the sample complexity significantly reduces.  This could suggest another form of ``forecast combination puzzle'': aggregation methods that ignore the correlations between experts could perform better than those take into account correlations, given a practical number of samples.  This phenomenon has been observed by empirical works \cite{makridakis_averages_1983, gupta_combination_1987, stock_combination_2004}.  Our results provide a rigorous theoretical explanation to this phenomenon. 


% % ===================================================

% % The role of \emph{prior} is important in the forecast aggregation problem. 
% % If we do not have any prior knowledge about the weather or the experts' predicting abilities, then the best we could do is basically some trivial aggregation methods, like taking the average of the experts' predictions, or simply guessing a constant $0.5$.\cite{arieli_robust_2018}. 
% % A natural approach, and in fact a standard approach to the forecast aggregation problem in the literature, is the data-driven approach. 
% % The idea is simple.  

 
% % In practice, we hardly have access to an accurate prior. 
% % A standard approach in the forecast aggregation literature to overcoming this issue is the data-driven approach. 
% % The idea is simple: since many forecasting tasks are repeated (like the weather forecasting example above), we can collect samples of experts' predictions and the outcomes of the predicted event, and use those samples to find a good aggregation method accordingly.  For example, one can use a weighted average where each expert's weight is determined by historical data.

% % This data-driven approach has in fact been a standard approach in the forecast aggregation literature, with numerous empirical works studying how well different aggregation methods work in different real-world forecasting tasks.  See Section~\ref{sec:related_works} for discussions.



% % However, in reality, especially in the weather forecasting example above, the forecasting task is repeated every day, and the outcome of the event being predicted is observed (rain or not).  So, one can observe the historical forecasting performance of each expert and adjust the aggregation method accordingly.  For example, one can use a weighted average aggregation method where each expert's weight is determined by empirical data of its performance.  This data-driven approach has in fact been a standard approach in the forecast aggregation literature, with numerous empirical works studying how well different aggregation methods work in different real-world forecasting tasks.  See Section~\ref{sec:related_works} for discussions.

\subsection{Related Works}\label{sec:related_works}

\paragraph{Data-driven aggregation}
Data-driven approaches to forecast aggregation date back to perhaps the first paper on forecast aggregation \cite{bates_combination_1969} and have been standard in the literature (see, e.g., surveys \cite{clemen_combining_1989, timmermann_chapter_2006} and more recent works \cite{yang_combining_2004, satopaa_combining_2014, babichenko_learning_2021, wang_forecast_2021, frongillo_efficient_2021, neyman2022no}).  
Many of these works focus on specific weighted average aggregators like \emph{linear pooling} (weighted arithmetic mean) \cite{yang_combining_2004} and \emph{logarithmic pooling} (normalized weighted geometric mean) \cite{satopaa_combining_2014, neyman2022no}, and the goal is to estimate the optimal weights from data, which can usually be solved by standard statistical tools.  
However, those weighted average aggregators are not necessarily the optimal \emph{Bayesian} aggregator unless the underlying distribution $P$ of signals and event satisfies some strict conditions (e.g., experts' forecasts are equal to the true probability of the event plus normally distributed noises \cite{winkler_combining_1981}).  For some distributions the performance of the Bayesian aggregator can be much better than the optimal weighted average. 
Our work aims to understand the sample complexity of Bayesian aggregation, namely how many samples are needed to approximate the Bayesian aggregator. %We think this is a fundamental question to a addressed.


Our work is closely related to a recent work \cite{babichenko_learning_2021} on Bayesian aggregation via \emph{online learning}.  For the case of conditionally independent experts, \cite{babichenko_learning_2021} shows that the Bayesian aggregator can be approximated with $\eps = \tilde O(n\sqrt T)$ regret.  By online-to-batch conversion (e.g., \cite{shalev-shwartz_online_2012}, Corollary 5.2), this implies a $T = \tilde O(\frac{n^2}{\eps^2})$ sample complexity upper bound for the batch learning setting.  Our paper studies the batch learning setting. For the conditional independence case, we obtain an improved bound of $\tilde O(\frac{1}{\eps^2})$.   
However, the loss function considered by \cite{babichenko_learning_2021} is different from ours: theirs is the logarithmic loss while ours is the squared loss.  Since the logarithmic loss is larger than the squared loss,
\yc{Is this comparison meaningful? We are comparing an unbounded loss function with a bounded loss function. Also, do you mean that the log loss is point-wise greater than the squared loss?}\tl{the log loss is point-wise greater than or equal to 2 times the squared loss, by Pinsker's inequality: $D_{KL}(p || q) = p \log\frac{p}{q} + (1-p)\log \frac{1-p}{1-q} \ge 2 |p - q|^2$.  So, if we get an $\eps$-optimal aggregator under log loss, then that is automatically an $\eps/2$-optimal aggregator for squared loss.  This implies that the sample complexity for the log loss is greater than or equal to the sample complexity for the squared loss, up to a constant factor. }\yc{Thanks! This is fine.}
their sample complexity bound should be greater than or equal to our bound.  We do not know whether there is a gap between the tight sample complexity bounds for the two loss functions. 


% \paragraph{Data-driven approaches to forecast aggregation and linear aggregation}
% Data-driven approaches to forecast aggregation already appeared in perhaps the first paper on forecast aggregation, \citet{bates_combination_1969}, and have been a standard practice in forecast aggregation (see, e.g., surveys by \citet{clemen_combining_1989} and \citet{timmermann_chapter_2006}). 
% Many of these works focus on weighted averaging, or more generally \emph{linear} aggregators, $f^{\bm \theta}(r_1, \ldots, r_n) = \sum_{i=1}^n \theta_i r_i + \theta_0$, studying how to use samples to estimate the best coefficient $\bm \theta$. 
% The use of linear aggregators is justified by the fact that the Bayesian optimal aggregator is indeed a linear function when the underlying distribution of experts' forecasts and the event satisfies some conditions, e.g., when experts' forecasts are the true probability of the event plus normally distributed noises (\citet{winkler_combining_1981}).
% While the restriction to linear aggregators and the assumption of normally distributed noise usually suffice for practical purposes, they do not necessarily capture the real underlying relationship between the event and the experts' forecasts.
% The Bayesian optimal aggregator is not linear in general, even for conditionally independent distributions (Section \ref{sec:conditionally_independent}).  
% Our work wants to understand how many samples are needed to approximately identify the Bayesian optimal aggregator.  We think this is a theoretically interesting and important question.
% Another reason why we do not restrict attentions to linear aggregators is that, once restricting to them, the aggregator learning problem reduces to a linear regression, and the sample complexity of aggregation becomes the sample complexity of linear regression, which is conceptually different from our purpose of understanding the sample complexity of aggregation \emph{itself}.
% While the sample complexity of linear aggregation has been studied by \citet{yang_combining_2004}, the sample complexity of Bayesian aggregation has not, as far as we know. 



\paragraph{Robust forecast aggregation}
Some recent works study the 
%There are also works on Bayesian aggregation that are not from a data-driven perspective
Bayesian aggregation problem \emph{not} from a data-driven perspective
\cite{frongillo_elicitation_2015, arieli_robust_2018, neyman_are_2021}.
In particular, \cite{arieli_robust_2018} and \cite{neyman_are_2021} study a ``robust forecast aggregation'' problem where the principal does not know and does not have samples from the prior distribution over experts' forecasts and the event.  They study the worst-case approximation ratio obtainable by a prior-free aggregator compared to the prior-aware Bayesian aggregator.  They obtain several negative results.  We are able to give positive results ($\eps$-approximation) because of two reasons: (1) we have sample access to the prior, and (2) the Bayesian aggregator benchmark they choose is in fact stronger than ours; see Section~\ref{sec:model} for a detailed discussion. 

% problem  (e.g., \cite{arieli_robust_2018, babichenko_learning_2021, neyman_are_2021}) than the traditional forecasting literature (e.g., \cite{bates_combination_1969, morris_combining_1977, winkler_combination_1983, clemen_combining_1989, timmermann_chapter_2006}).
% The latter works usually assume a parametric family of distributions over the the ground truth and the experts' predictions.  Then, the learning task boils down to the estimation of parameters using historical data.

% Non-Bayesian approach: \cite{bates_combination_1969, newbold_experience_1974, winkler_combination_1983, granger_improved_1984}.
% Survey: \cite{clemen_combining_1989, timmermann_chapter_2006}. 

% \paragraph{No-regret learning}
% (e.g., \cite{cesa-bianchi_prediction_2006, frongillo_efficient_2021}) 

% Aggregating forecasts is different from aggregating signals \cite[p.198-199]{granger_improved_1984} \cite[p.168-169]{granger_invited_1989}, \cite[p.143]{timmermann_chapter_2006}. 

% Works about \emph{recalibration} (e.g., \cite{turner_forecast_2014, budescu_identifying_2015}) also study how to choose aggregators based on experts' historical performance.  But those works are mainly empirical: they evaluate the performance of specific aggregator-choosing schemes based on real-world data, without sample complexity analysis.  

\paragraph{Sample complexity of mechanism design}  Our work may remind the reader of a long line of research on the sample complexity of mechanism design, in particular revenue maximization (e.g., \cite{cole_sample_2014, dhangwatnotai_revenue_2015, morgenstern_pseudo-dimension_2015, devanur_sample_2016, balcan_sample_2016, cai_learning_2017, guo_settling_2019, brustle_multi-item_2020, gonczarowski_sample_2021, guo_generalizing_2021}).  A key observation from these works is that, the number of samples needed to learn an $\eps$-optimal auction for $n\ge 1$ independent bidders is increasing in $n$, because when there are more bidders, although we can obtain higher revenue, the optimal auction benchmark is also improved.  We see a similar phenomenon that the sample complexity increases with the number of experts in the forecast aggregation problem  in the general case, but not in the case where experts are conditionally independent. 



==> intro_v6.tex <==
\section{Introduction} 
Suppose you want to know whether it will rain tomorrow.  A Google search on ``weather'' returns 40\% probability of raining for tomorrow. The weather forecasting app on your phone shows 85\%.  And one of your friends, who is an expert in meteorology, predicts 65\%.  How do you aggregate these different predictions into a single, accurate prediction?  
This problem is called \emph{forecast aggregation} or \emph{forecast combination} \cite{bates_combination_1969, clemen_combining_1989, timmermann_chapter_2006}.
It has innumerable applications in fields ranging from economics, statistics, operations research, to machine learning, decision theory, and of course, climate science. 

\yc{Tao, could you please fill in the missing citations and also check whether I put the references at the appropriate places?}
% A known phenomenon in many empirical works on forecast aggregation is the ``forecast combination puzzle'' \cite[p.428]{stock_combination_2004}: a simple aggregation methods like the unweighted averaging of all experts' forecasts often outperform more sophisticated, data-driven, aggregation methods. 

A straightforward solution to forecast aggregation is to simply take the (unweighted) average of all experts' forecasts. Simple as it is, unweighted average performs surprisingly well in practice, as observed by many forecast aggregation works from 1960s to 2020s (e.g., \cite{bates_combination_1969, newbold_experience_1974, makridakis_averages_1983, gupta_combination_1987, clemen_combining_1989, timmermann_chapter_2006, makridakis_m4_2020}). 
Naturally, when past data of expert forecasts and event outcomes (e.g., historical weather forecasts and outcomes) are available, one may hope to leverage on such data to learn more accurate aggregators. While adjusting weights of experts in averaging according to their individual historical accuracy has led to improved accuracy for the aggregated prediction~\cite{winkler_combination_1983}, interestingly,
% more sophisticated data-driven aggregation methods, including accounting for correlation of experts when setting their weights \cite{winkler_combination_1983} and training neural network aggregators []
\yc{I wonder whether a more ML example is better} 
\tl{maybe we should not mention neural networks here.  I didn't find evidence showing that neural networks aggregators are worse than simple average. }
more sophisticated data-driven methods like adjusting the weights using ordinary least squared regression \cite{genre_combining_2013} and covariance estimation \cite{makridakis_averages_1983, winkler_combination_1983} were often outperformed by the unweighted average.
%\cite{gupta_combination_1987, stock_combination_2004, genre_combining_2013}.
The dominance of simple aggregators over more sophisticated data-driven methods is observed so often in empirical applications that it is termed ``the forecast combination puzzle'' \cite[p.428]{stock_combination_2004}.

%This ‘forecast combination puzzle’—the repeated finding that simple combination forecasts outperform sophisticated adaptive combination methods in empirical appli- cations

There are many potential explanations for the forecast combination puzzle~\cite{smith_simple_2009, genre_combining_2013, claeskens_forecast_2016}. In some scenarios, the past events are different from the future events in fundamental ways (e.g., geopolitical forecasting) and hence past data may not be informative in predicting the future. Another widely accepted conjecture is that the amount of past data is not large enough for a data-intensive method to % learn an accurate aggregator.
perform well.
% Indeed, the sample sizes in works that support the simple average are small under today's ``big-data'' standard (24 in \cite{granger_improved_1984}, 69 in \cite{satopaa_combining_2014},87 in \cite{baron_two_2014}, 100 in \cite{gupta_combination_1987}).
Indeed, the sample sizes in many empirical forecast aggregation works are small under today's ``big-data'' standard (24 in \cite{granger_improved_1984}, 69 in \cite{satopaa_combining_2014}, 87 in \cite{baron_two_2014}, 100 in \cite{gupta_combination_1987}).
However, there are aggregation settings where it is reasonable to think that future events are similar to past events and we do have abundant data --- 
%for instance, weather forecasting and some forecasting competitions on Kaggle\footnote{\url{https://www.kaggle.com/c/m5-forecasting-accuracy}}. Such settings are well-suited for data-driven methods.
for instance, the forecasting of weather, stock prices \cite{donaldson_forecast_1996}, and some forecasting competitions on Kaggle\footnote{\url{https://www.kaggle.com/c/m5-forecasting-accuracy}}. Such settings are well-suited for data-driven methods.
In fact, when given enough data, neural network based nonlinear aggregators can perform better than traditional linear aggregators \cite{donaldson_forecast_1996, ming_shi_improving_1999, wang_optimal_2018}.
\tl{Added citations for neural network aggregators}
It's hence tempting to ask \emph{how many} data are needed for data-driven aggregators to achieve high accuracy in these settings. 

\yc{In the current version, I didn't talk about overfitting. Is it ok to omit it? Maybe we can find a different place to cite \cite{smith_simple_2009, genre_combining_2013, claeskens_forecast_2016}.}
\tl{I think it's OK to omit it.  And just put them after the first sentence ``there are many potential explanations xxx''? }\yc{OK. Added the citations.}

In this paper, we initiate the study of \emph{sample complexity of forecast aggregation}, building upon a standard Bayesian forecasting model \cite{morris_decision_1974, winkler_combining_1981, geweke_chapter_2006}.
\tl{Add brief description of the model}
In this model, the optimal aggregator (which is Bayesian) depends on an underlying unknown joint distribution of the experts' reports and the event outcome, from which we obtain samples.  
\tl{I'm a bit confused by the two ``models'' here.  Maybe no need to say ``in a statistical learning model''? } \yc{I removed statistical learning model. The batch learning perspective, that is, we have samples and want to learn an aggregator, is what I mean by a statistical learning model. I don't think the standard Bayesian forecasting model has the learning aspect.}
We ask:
\begin{center}
    \emph{How many samples do we need to approximately learn the optimal Bayesian aggregator?}
\end{center} 
We show that the sample complexity of forecast aggregation can be extremely large in the worst case. But it is significantly lower for some special families of distributions. \tl{Should we say information structure or distributions?}\yc{Changed it to distributions for consistency.}
Our results provide partial explanation for the observed forecast combination puzzle. 

\paragraph{Our results and techniques} 
In our model, there are $n$ experts and one principal. Each expert $i$ observes a private signal $s_i \in \S_i$ about an unknown binary event (state of the world) $\omega\in \Omega = \{0, 1\}$. Experts' signals and the event jointly follow an underlying distribution $P$. Each expert reports its posterior belief $r_i = P(\omega = 1 \,|\, s_i)$ about $\omega$ to the principal, who then aggregates all the reports $r_1, \ldots, r_n$ into a single prediction for $\omega$.
The principal does not know $P$ but has i.i.d.~``samples'' from it, where each sample is a tuple
of experts' reports (not signals) and the realization of the event. Using these samples, the principal aims to find an aggregator $\hat f: [0, 1]^n \to [0, 1]$ that is ``$\eps$-close'' to the Bayesian optimal aggregator $f^*$ defined by $f^*(r_1, \ldots, r_n) = P(\omega = 1 \,|\, r_1, \ldots, r_n)$, where ``$\eps$-closeness'' is measured in the mean squared difference: $\E_P\big[|\hat f(r_1, \ldots, r_n) - f^*(r_1, \ldots, r_n)|^2\big]\le \eps$. 

Assuming a finite signal space of size $|\S_i| = m$ for each expert, we show that: 
\begin{itemize}
    \item To find an aggregator $\hat f$ that is $\eps$-close to the optimal aggregator $f^*$ with high probability for any distribution $P$, $\tilde O(\frac{m^{n}}{\eps^2})$ samples are sufficient, and $\tilde \Omega(\frac{m^{n-2}}{\eps})$ samples are necessary.\footnote{The $\tilde O(\cdot)$ and $\tilde \Omega(\cdot)$ notations omit logarithmic factors.} (Theorem~\ref{thm:general_distribution_both}.)
\end{itemize}

The exponential sample complexity lower bound $\tilde \Omega(\frac{m^{n-2}}{\eps})$ implies that the optimal aggregator $f^*$ is rather difficult to learn, and significantly more difficult when the number of experts increases.

Both the upper bound $\tilde O(\frac{m^{n}}{\eps^2})$ and the lower bound $\tilde \Omega(\frac{m^{n-2}}{\eps})$ are proved by reductions to the \emph{distribution learning} problem.  We note that the optimal aggregator $f^*$ is completely determined by the joint probabilities of reports and event $P(r_1, \ldots, r_n, \omega)$ induced by $P$. 
If we can learn the unknown distribution $P$ well from samples, then we are able to approximate $f^*$ well.  Since $P$ has a finite support of size $2m^n$ and learning distributions with support size $2m^n$ in total variation distance $\eps_{\TV}$ requires at most $\tilde O(\frac{m^n}{\eps_{\TV}^2})$ samples, we obtain the claimed upper bound. 

The proof of the lower bound, however, is tricky.
We first note that the opposite reduction also holds: if we can approximate $f^*$ well, then we can estimate $P$ well.  Then, one may expect that the known lower bound $\tilde \Omega(\frac{m^n}{\eps_{\TV}^2})$ for learning distributions with support size $2m^n$ within total variation distance $\eps_{\TV}$ should apply here.  However, that lower bound does not apply directly because in our setting the samples of experts' reports $r_i^{(t)} = P(\omega = 1 \,|\, s_i^{(t)})$ contain information about the probability densities of $P$, while in the traditional distribution learning setting the samples themselves do not contain any information about the probability densities (only the empirical frequency of samples contains that information).  The additional information contained in $r_i^{(t)}$ can reduce the sample complexity of distribution learning.  So, to prove our lower bound we restrict attentions to a special family $\mathcal P$ of distributions where all the $P$'s in $\mathcal P$ share the same marginal conditional distribution $P(s_i \,|\, \omega)$ for each expert (yet the joint conditional distribution $P(s_1, \ldots, s_n \,|\, \omega)$ is different for different $P$), so each expert's sample of report $r_i^{(t)}$ contains no ``useful'' information about $P$.  This reduces to the problem of learning a family $\mathcal D$ of joint distributions (over the joint signal space $\bm \S = \S_1 \times \cdots \times \S_n$) that share the same marginal $D(s_i) = D'(s_i)$ but have different joint probabilities $D(\bm s) \ne D'(\bm s)$.
We prove a sample complexity lower bound of $\Omega(\frac{m^{n-2}}{\eps_{\TV}^2})$ for this special distribution learning problem, which gives the lower bound for the forecast aggregation problem. 

As indicated by the above intuition, the exponentially large sample complexity of forecast aggregation stems from the fact that we need to estimate the correlation between experts, namely, to estimate the joint probability $P(s_1, \ldots, s_n \, | \, \omega)$ besides the marginal $P(s_i \, | \, \omega)$. 
% This requires a large number of samples.
This motivates us to study the special case where (the signals of) experts are conditionally independent, namely, $s_i$'s are independent conditioned on $\omega$. 
The sample complexity is significantly reduced in this case:
\begin{itemize}
    \item If experts are conditionally independent, then an $\eps$-optimal aggregator $\hat f$ can be found with high probability using only $\tilde O(\frac{1}{\eps^2})$ samples.  $\tilde \Omega(\frac{1}{\eps})$ samples are necessary. (Theorem~\ref{thm:conditionally_independent_general}.)
\end{itemize}

Surprisingly, the sample complexity upper bound $\tilde O(\frac{1}{\eps^2})$ does not depend on the number of agents $n$ or the signal space size $m$.
The reason is that, in the conditional independence case, the optimal aggregator $f^*$ takes a simple form: $f^*(\bm r) = \frac{1}{1 + (\frac{p}{1-p})^{n-1} \prod_{i=1}^n \frac{1-r_i}{r_i}}$, where $p = P(\omega = 1)$ is the prior probability of $\omega = 1$. 
This allows us to focus only on the class of aggregators of the form  $\mathcal F = \big \{ f^\theta : f^\theta(\bm r) = \frac{1}{1 + \theta^{n-1} \prod_{i=1}^n \frac{1-r_i}{r_i}} \big \}$.  We show that the \emph{pseudo-dimension} of the loss functions associated with this class of aggregators is upper bounded by $d = O(1)$.  By known results in statistical learning theory (e.g., \cite{anthony_neural_1999}), this implies that an $\eps$-optimal aggregator can be learned with $\tilde O(\frac{d}{\eps^2}) = \tilde O(\frac{1}{\eps^2})$ samples, which proves the upper bound. 
The lower bound $\tilde \Omega(\frac{1}{\eps})$ is proved by a non-trivial reduction from the \emph{distinguishing distributions} problem. 

We then try to close the gap between $\tilde O(\frac{1}{\eps^2})$ and $\tilde \Omega(\frac{1}{\eps})$ for the conditional independence case by investigating two special cases where the experts are either ``very informative'' or ``very non-informative''.  In both cases the upper bound can be improved to $\tilde O(\frac{1}{\eps})$ (Theorem~\ref{thm:strongly-informative-upper-bound} and \ref{thm:weakly-informative-upper-bound:new}).

Finally, in Section~\ref{sec:multi-outcome-events} we generalize our model from binary events to multi-outcome events and obtain sample complexity bounds that depend on the size of the outcome space $|\Omega|$.

% In the remainder of the paper, we first discuss related works in Section~\ref{sec:related_works}.  Section~\ref{sec:model} introduces our model and preliminaries. Section~\ref{sec:general_distribution} studies the sample complexity for general distributions.  Section~\ref{sec:conditionally_independent} focuses on the conditional independence case.  We conclude and discuss future directions in Section~\ref{sec:conclusion}. 
 

% \subsection{Overview of Our Results}
% \paragraph{Model} 
% To formalize the sample complexity question above, we consider the following forecast aggregation model, which is a Bayesian framework proposed by Morris (1974) \cite{morris_decision_1974} and more recently studied by \cite{arieli_robust_2018, babichenko_learning_2021, neyman_are_2021}: A principal wants to predict the unknown state of the world $\omega \in \{0, 1\}$.  There are $n$ experts, each observing a private signal $s_i \in \S_i$ that correlates with the state of the world according to some underlying distribution $P$.  Experts know (their marginals of) the distribution $P$ and report their posterior beliefs about $\omega$ to the principal: $r_i = P(\omega = 1 \mid s_i)$.  Given the reports $\bm r = (r_1, \ldots, r_n)$, the principal aggregates them into a single prediction $f(r_1, \ldots, r_n) \in [0, 1]$.  Crucially, we assume that the distribution $P$ is unknown to the principal and can be arbitrarily chosen.  If the principal knows $P$, then it can aggregate ``optimally'' (we formally define ``optimality'' in Section~\ref{sec:model}) using the Bayes' rule: compute the posterior probability of $\omega = 1$ given all the information it receives, $f^*(r_1, \ldots, r_n) = P(\omega = 1 \mid r_1, \ldots, r_n)$.

% The principal has access to $T$ i.i.d.~samples of reports and the realization of the state of the world according to $P$: 
% \begin{equation*}
%     (\bm r^{(1)}, \omega^{(1)}), (\bm r^{(2)}, \omega^{(2)}), ~ \ldots, ~ (\bm r^{(T)}, \omega^{(T)}),  \quad \quad \bm r^{(t)} = (r_1^{(t)}, \ldots, r_n^{(t)}),  
% \end{equation*}
% using which it finds an aggregator $\hat f: [0, 1]^n \to [0, 1]$. 
% An aggregator is $\eps$-optimal if its mean squared difference with $f^*$ is less than $\eps$, where the mean is with respect to $P$: $\E_P\big[|f(\bm r) - f^*(\bm r)|^2\big]\le \eps$. 
% Now, the sample complexity question can be rephrased as follows: 
% \begin{center}
% \emph{How many samples are necessary and sufficient for finding an $\eps$-optimal aggregator \\
% (with high probability over the random draw of samples)?} 
% \end{center}

% \paragraph{Results}
% Unlike many forecast aggregation works that restrict attentions to linear aggregators $\hat f(\bm r) = \sum_{i=1}^n a_i r_i$, we do not put such restrictions on $\hat f$, because we want to approximate the optimal aggregator $f^*$ which need not be linear.  However, such approximation cannot be done with a finite number of samples if $P$ can be an arbitrary continuous distribution.  Hence, our work makes two types of assumptions on $P$: (1) \emph{discrete signal space}: each $\S_i$ is a finite set of size $m < \infty$; (2) \emph{conditionally independent signals}: $s_1, \ldots, s_n$ are independently distributed conditioning on $\omega$.  We prove that, under these assumptions, an $\eps$-optimal aggregator can be found with a finite number of samples.  Specifically, the number of samples is upper bounded by: 
% \begin{itemize}
%     \item Discrete signal space: $O\big(\frac{m^n}{\eps^2}\big)$ (Theorem~\ref{thm:general_distribution_upper_bound}). 
%     \item Conditionally independent signals: $O\big(\frac{(n-1)^2}{\rho \eps}\big)$, where $\rho = \frac{P(\omega = 1)}{P(\omega = 0)}$ is a constant (Theorem~\ref{thm:conditionally_independent_upper_bound}). 
% \end{itemize}

% The above two results answer the ``sufficient'' part in the question we raised above.  The more interesting, and more challenging, part is how many samples are ``necessary''?  We show that, in order to obtain $\eps$-optimal aggregators with high probability, one needs at least the following numbers of samples: 
% \begin{itemize}
%     \item Discrete signal space: $\Omega\big(\frac{m^{n-2}}{\eps}\big)$ (Theorem~\ref{thm:general_distribution_lower_bound}). 
%     \item Conditionally independent signals: $\Omega\big(\frac{1}{\eps}\big)$ (Theorem~\ref{thm:conditionally_independent_lower_bound}). 
% \end{itemize}

% \paragraph{Discussion}
% The exponential sample complexity of learning $\eps$-optimal aggregators for distributions over discrete signal space basically means that learning the optimal aggregator is rather difficult.  As we show in the proof, this difficulty stems from the fact that we need to estimate the correlations between experts.  To estimate such correlations with ``$\eps$-accuracy'', we need $\Omega\big(\frac{m^{n-2}}{\eps}\big)$ samples.
% In practice, this number of samples can hardly be obtained.

% However, once we assume that experts are conditionally independent, the sample complexity significantly reduces.  This could suggest another form of ``forecast combination puzzle'': aggregation methods that ignore the correlations between experts could perform better than those take into account correlations, given a practical number of samples.  This phenomenon has been observed by empirical works \cite{makridakis_averages_1983, gupta_combination_1987, stock_combination_2004}.  Our results provide a rigorous theoretical explanation to this phenomenon. 


% % ===================================================

% % The role of \emph{prior} is important in the forecast aggregation problem. 
% % If we do not have any prior knowledge about the weather or the experts' predicting abilities, then the best we could do is basically some trivial aggregation methods, like taking the average of the experts' predictions, or simply guessing a constant $0.5$.\cite{arieli_robust_2018}. 
% % A natural approach, and in fact a standard approach to the forecast aggregation problem in the literature, is the data-driven approach. 
% % The idea is simple.  

 
% % In practice, we hardly have access to an accurate prior. 
% % A standard approach in the forecast aggregation literature to overcoming this issue is the data-driven approach. 
% % The idea is simple: since many forecasting tasks are repeated (like the weather forecasting example above), we can collect samples of experts' predictions and the outcomes of the predicted event, and use those samples to find a good aggregation method accordingly.  For example, one can use a weighted average where each expert's weight is determined by historical data.

% % This data-driven approach has in fact been a standard approach in the forecast aggregation literature, with numerous empirical works studying how well different aggregation methods work in different real-world forecasting tasks.  See Section~\ref{sec:related_works} for discussions.

% % However, in reality, especially in the weather forecasting example above, the forecasting task is repeated every day, and the outcome of the event being predicted is observed (rain or not).  So, one can observe the historical forecasting performance of each expert and adjust the aggregation method accordingly.  For example, one can use a weighted average aggregation method where each expert's weight is determined by empirical data of its performance.  This data-driven approach has in fact been a standard approach in the forecast aggregation literature, with numerous empirical works studying how well different aggregation methods work in different real-world forecasting tasks.  See Section~\ref{sec:related_works} for discussions.

\subsection{Related Works}\label{sec:related_works}

\paragraph{Data-driven aggregation}
Data-driven approaches to forecast aggregation date back to perhaps the first paper on forecast aggregation \cite{bates_combination_1969} and have been a standard practice in the literature (see, e.g., surveys \cite{clemen_combining_1989, timmermann_chapter_2006} and more recent works \cite{yang_combining_2004, satopaa_combining_2014, babichenko_learning_2021, wang_forecast_2021, frongillo_efficient_2021, neyman2022no}).  
Many of these works focus on specific weighted average aggregators like \emph{linear pooling} (weighted arithmetic mean) \cite{yang_combining_2004} and \emph{logarithmic pooling} (normalized weighted geometric mean) \cite{satopaa_combining_2014, neyman2022no}, and the goal is to estimate the optimal weights from data, which can usually be solved by standard statistical tools.  
However, those weighted average aggregators are not necessarily the optimal \emph{Bayesian} aggregator unless the underlying distribution $P$ of signals and event satisfies some strict conditions (e.g., experts' forecasts are equal to the true probability of the event plus normally distributed noises \cite{winkler_combining_1981}).  For some distributions the performance of the Bayesian aggregator can be much better than the optimal weighted average. 
Our work aims to understand the sample complexity of Bayesian aggregation, namely how many samples are needed to approximate the Bayesian aggregator. %We think this is a fundamental question to a addressed.


Our work is closely related to a recent work \cite{babichenko_learning_2021} on Bayesian aggregation via \emph{online learning}.  For the case of conditionally independent experts, \cite{babichenko_learning_2021} shows that the Bayesian aggregator can be approximated with $\eps = \tilde O(n\sqrt T)$ regret.  By online-to-batch conversion (e.g., \cite{shalev-shwartz_online_2012}, Corollary 5.2), this implies a $T = \tilde O(\frac{n^2}{\eps^2})$ sample complexity upper bound for the batch learning setting.  Our paper studies the batch learning setting. For the conditional independence case, we obtain an improved bound of $\tilde O(\frac{1}{\eps^2})$.   
However, the loss function in \cite{babichenko_learning_2021} is different from ours: theirs is the logarithmic loss while ours is the squared loss.  Since the logarithmic loss is larger than the squared loss,
\yc{Is this comparison meaningful? We are comparing an unbounded loss function with a bounded loss function. Also, do you mean that the log loss is point-wise greater than the squared loss?}\tl{the log loss is point-wise greater than or equal to 2 times the squared loss, by Pinsker's inequality: $D_{KL}(p || q) = p \log\frac{p}{q} + (1-p)\log \frac{1-p}{1-q} \ge 2 |p - q|^2$.  So, if we get an $\eps$-optimal aggregator under log loss, then that is automatically an $\eps/2$-optimal aggregator for squared loss.  This implies that the sample complexity for the log loss is greater than or equal to the sample complexity for the squared loss, up to a constant factor. }\yc{Thanks! This is fine.}
their sample complexity bound should be greater than or equal to our bound.  We do not know whether there is a gap between the tight sample complexity bounds for the two loss functions. 


% \paragraph{Data-driven approaches to forecast aggregation and linear aggregation}
% Data-driven approaches to forecast aggregation already appeared in perhaps the first paper on forecast aggregation, \citet{bates_combination_1969}, and have been a standard practice in forecast aggregation (see, e.g., surveys by \citet{clemen_combining_1989} and \citet{timmermann_chapter_2006}). 
% Many of these works focus on weighted averaging, or more generally \emph{linear} aggregators, $f^{\bm \theta}(r_1, \ldots, r_n) = \sum_{i=1}^n \theta_i r_i + \theta_0$, studying how to use samples to estimate the best coefficient $\bm \theta$. 
% The use of linear aggregators is justified by the fact that the Bayesian optimal aggregator is indeed a linear function when the underlying distribution of experts' forecasts and the event satisfies some conditions, e.g., when experts' forecasts are the true probability of the event plus normally distributed noises (\citet{winkler_combining_1981}).
% While the restriction to linear aggregators and the assumption of normally distributed noise usually suffice for practical purposes, they do not necessarily capture the real underlying relationship between the event and the experts' forecasts.
% The Bayesian optimal aggregator is not linear in general, even for conditionally independent distributions (Section \ref{sec:conditionally_independent}).  
% Our work wants to understand how many samples are needed to approximately identify the Bayesian optimal aggregator.  We think this is a theoretically interesting and important question.
% Another reason why we do not restrict attentions to linear aggregators is that, once restricting to them, the aggregator learning problem reduces to a linear regression, and the sample complexity of aggregation becomes the sample complexity of linear regression, which is conceptually different from our purpose of understanding the sample complexity of aggregation \emph{itself}.
% While the sample complexity of linear aggregation has been studied by \citet{yang_combining_2004}, the sample complexity of Bayesian aggregation has not, as far as we know. 



\paragraph{Robust forecast aggregation}
Some recent works study the 
%There are also works on Bayesian aggregation that are not from a data-driven perspective
Bayesian aggregation problem \emph{not} from a data-driven perspective
\cite{frongillo_elicitation_2015, arieli_robust_2018, neyman_are_2021}.
In particular, \cite{arieli_robust_2018} and \cite{neyman_are_2021} study a ``robust forecast aggregation'' problem where the principal does not know and does not have samples from the prior distribution over experts' forecasts and the event.  They study the worst-case approximation ratio obtainable by a prior-free aggregator compared to the prior-aware Bayesian aggregator.  They obtain several negative results.  We are able to give positive results ($\eps$-approximation) because of two reasons: (1) we have sample access to the prior, and (2) the Bayesian aggregator benchmark they choose is in fact stronger than ours; see Section~\ref{sec:model} for a detailed discussion. 

% problem  (e.g., \cite{arieli_robust_2018, babichenko_learning_2021, neyman_are_2021}) than the traditional forecasting literature (e.g., \cite{bates_combination_1969, morris_combining_1977, winkler_combination_1983, clemen_combining_1989, timmermann_chapter_2006}).
% The latter works usually assume a parametric family of distributions over the the ground truth and the experts' predictions.  Then, the learning task boils down to the estimation of parameters using historical data.

% Non-Bayesian approach: \cite{bates_combination_1969, newbold_experience_1974, winkler_combination_1983, granger_improved_1984}.
% Survey: \cite{clemen_combining_1989, timmermann_chapter_2006}. 

% \paragraph{No-regret learning}
% (e.g., \cite{cesa-bianchi_prediction_2006, frongillo_efficient_2021}) 

% Aggregating forecasts is different from aggregating signals \cite[p.198-199]{granger_improved_1984} \cite[p.168-169]{granger_invited_1989}, \cite[p.143]{timmermann_chapter_2006}. 

% Works about \emph{recalibration} (e.g., \cite{turner_forecast_2014, budescu_identifying_2015}) also study how to choose aggregators based on experts' historical performance.  But those works are mainly empirical: they evaluate the performance of specific aggregator-choosing schemes based on real-world data, without sample complexity analysis.  

\paragraph{Sample complexity of mechanism design}  Our work may remind the reader of a long line of research on the sample complexity of revenue maximization in mechanism design (e.g., \cite{cole_sample_2014, dhangwatnotai_revenue_2015, morgenstern_pseudo-dimension_2015, devanur_sample_2016, balcan_sample_2016, cai_learning_2017, guo_settling_2019, brustle_multi-item_2020, gonczarowski_sample_2021, yang_learning_2021, guo_generalizing_2021}).  In particular, \cite{guo_generalizing_2021} gives a general framework to bound the sample complexity for mechanism design problems that satisfy a ``strong monotonicity'' property, but this property is not satisfied by our forecast aggregation problem.  A key observation from this line of works is that, the number of samples needed to learn an $\eps$-optimal auction for $n\ge 1$ independent bidders is increasing in $n$, because when there are more bidders, although we can obtain higher revenue, the optimal auction benchmark is also improved.  We see a similar phenomenon that the sample complexity of forecast aggregation increases with the number of experts in the general case, but not in the case where experts are conditionally independent. 


